PARQO: Penalty-Aware Robust Plan Selection in Query Optimization

The effectiveness of a query optimizer relies on the accuracy of selectivity estimates. The execution plan generated by the optimizer can be extremely poor in reality due to uncertainty in these estimates. This paper presents PARQO (Penalty-Aware Robust Plan Selection in Query Optimization), a novel system where users can define powerful robustness metrics that assess the expected penalty of a plan with respect to true optimal plans under uncertain selectivity estimates. PARQO uses workload-informed profiling to build error models, and employs principled sensitivity analysis techniques to identify human-interpretable selectivity dimensions with the largest impact on penalty. Experiments on three benchmarks demonstrate that PARQO finds robust, performant plans, and enables efficient and effective parametric optimization.

==> 1-intro-old.tex <==
The idea of \emph{robust query optimization} has been around for years~\cite{chu1999least, chaudhuri2010variance, jayant2008identifying}.
Many different notions of robustness and approaches for finding robust plans have been introduced (see~\Cref{sec:related} for more discussion).
To illustrate the intricacies in modeling robustness and how our work differs from previous work,
consider two questions:
\begin{enumerate}[leftmargin=*]
    \item How much weight do we put on extreme errors in selectivity estimates that may be unlikely given by database workload?
    Are we willing to sacrifice considerable average-case performance?
    \item Say we have a big error in some selectivity estimate, but does it matter in the end?
    Considering that this error might affect the estimated costs of many candidate plans in similar ways, will it actually alter the optimal plan choice?
    And even if it does lead to a suboptimal plan, is its cost far off from the optimal?
\end{enumerate}
There are perhaps no single ``correct'' answers to these questions.
Our system, \emph{\textbf{\OurSys}} (\emph{\textbf{P}enalty-\textbf{A}ware \textbf{R}obust \textbf{Q}uery \textbf{O}ptimization}),
answers them as follows.
First, \OurSys\ believes that treating all errors as equally likely often leads to over-conservative decisions,
so it takes the general approach of \emph{stochastic optimization}~\cite{spall2005introduction},
using a statistical model of the selectivity estimation errors that reflects the database workload.
Second, \OurSys\ believes that ``what matters'' depends on the application scenario,
and that many scenarios require us to define robustness in more nuanced ways,
such as in terms of a \emph{penalty} relative to the optimal plan had we known true selectivities.
This penalty in general depends on the cost difference
(and to capture different levels of risk tolerance, may be nonlinear in the cost difference).
Relating this answer back to our answer to the first question,
a robust plan should minimize the \emph{expected} penalty
under an error model reflecting the database workload,
for the user-defined penalty function.
To the best of our knowledge, \OurSys\ is the first system with this combination of answers to the above questions.
As will be discussed in \Cref{sec:related}, previous work either does not follow a stochastic optimization approach,
or chooses less general robustness measures (and/or employs heuristics reflecting such objectives)
that depend only on an individual plan (e.g., whether its own cost is sensitive to the error)
but not how it compares with other candidates (such as the true optimal).

More specifically, \OurSys\ makes the following contributions.
\begin{itemize}[leftmargin=*]
    \item First, we formalize robustness as \emph{expected penalty},
    where the key components in this definition include
    a conditional error distribution,
    which we show how to obtain by profiling the database workload,
    and a penalty function,
    which can assess ``regret'' with respect to the true optimal.
    This powerful combination allows \OurSys\ to tailor to a broader range of application needs.
    \item Real queries often contain many joining tables and predicates;
    for example, in the JOB benchmark~\cite{job} based on a real dataset (IMDB),
    query Q29 joins 17 tables, and the PostgreSQL optimizer makes more than 13{,}000 cardinality estimates when optimizing this query.
    Such high dimensionality makes the problem of robust query optimization very challenging.
    As with previous work, we must reduce dimensionality to tame complexity.
    Existing heuristics for selecting dimensions are not always aligned to the definition of robustness,
    and methodically, they rely on rather rudimentary techniques that analyze dimensions one at a time.
    We identify principled techniques from the \emph{sensitivity analysis} literature~\cite{saltelli2010variance, wainwright2014making}
    that account for interactions among multiple dimensions,
    and apply them to our setting.
    Our selection of \emph{sensitive dimensions} considers the given expected penalty objective,
    and therefore is fully aware of and tailored to the error distribution as well as the penalty definition.
    Finally, selected sensitive dimensions correspond to selection/join condition combinations in the query,
    which are interpretable and actionable --- for example,
    a user may investigate a sensitive dimension and improve its accuracy \revb{(by selectively reanalyzing statistics and/or sampling)} in order to obtain a better plan.
    \item Given a query and its selectivity estimates, we show how to find a robust plan that minimizes expected penalty,
    focusing on the sensitive dimensions.
    Except for very expensive queries, the amount of work that goes into finding a robust plan from end to end
    (including the identification of sensitive dimensions through sensitivity analysis) may not
    justify doing so to optimize just a single execution.
    We show how to reuse the work in robust query optimization and amortize its cost 
    in the setting of \emph{parametric query optimization} (\emph{PQO})~\cite{ioannidis1997parametric},
    where the optimization overhead is shared among multiple queries with the same template but different query parameters,
    which frequently arise in practice.
    \item \common{\OurSys\ is designed to work with existing optimizers and cardinality estimation methods.
    We have implemented it on top of PostgreSQL and conducted an end-to-end evaluation using three popular benchmarks: JOB~\cite{job}, DSB~\cite{ding2021dsb}, and STATS-CEB~\cite{han2021cardinality}.}
    We demonstrate how \OurSys\ is able to suggest hints that are interpretable and actionable for understanding and improving query performance,
    how resilient \OurSys's robust plans are against inaccurate selectivity estimates and how they soundly outperform traditional plans,
    and finally, how \OurSys\ delivers significant benefits to multiple queries in the PQO setting.
    We illustrate \OurSys's effectiveness in these scenarios using an example below.
\end{itemize}

==> 10-more.tex <==
R3R1/O1/D1
    [1] basically is looking for \% best. uses samples at runtime to get distributions of the selectivity. quantile.
    first, needs to runtime sampling approach, which requires deep DBMS support can is not used except for very expensive queries.
    the quantile thing is fixed and limited... not flexible.\\
    thank for pointing out 2... we were not aware before.  [2] matches our motivation on a high level. We propose an approach that is capable of producing the execution time distribution for plans, which they call the Execution Time Distribution Constructor (ET). importnatly, it uses conformal prediction to learn how to take a very specific plan and predict distribution of execution time. this must be done by lots of training????? (not clear)  then it enuemrates several candidate plans (BAO-style, inject various hints) and compare the distribution to be pick one, using the object pick highest probability to complete under threshodl time (very simple, basically not relative). variants try to pick plans for a set of plans to meet overall threashold objectve on total completeions time or \% of query completed. key differences: they don't offer anything explanable... no attribution of error to dimensions. we have much more flexible objective.
    it would be difficult to predict whether ours will stick, and we doubt there is a silver bullet to make industry adopt, but we note there are some issues that we think affects applicability of previous approcaches.
    that we have taken care to correct. (we tried best to make as little assumption about inner workings as possible, only assume opt and cost; flexibility and explicitly definable opitmization goal) hence, we hope it's a good direction.}
    \textcolor{red}{****[[[[Haibo: 1. This work is based on BAO, changing from predicting a single value of the execution time to a distribution. They focus on improving the mapping relation between "query plan" to "execution time" by learning from real executions. (So in some sense they ignore weather the cardinality estimation is accurate or not.) In contrast, we analyze cardinality errors and their sensitivities, ensuring our plan selection is resistant to these uncertainties. 2. same as BAO, the plan set construction method using some high-level hints, which is naive and maybe overlook those real robust plan. The plan choice is also not explainable and hence can not demonstrate any robustness. 3. To feature each plan as a vector, they rely on the default cardinality estimation which overlook the possible uncertainty and their penalty. 4. To build the training set, they need to additionally execute every candidate plan for each query in the workload, which is significantly time-consuming.]]]]****


R5D8

\revc{discuss additionally as related work! analytically deriving optimality range is nice, but not clear how they allow for tolerance --- in this regard they don't really expose more plan choices for robust plans that are hidden below the lower envelop.
also they make much stronger assumptions about the innerworkings of an optimzer to do this... if we relax this assumption, we can improve on our sampling.} \haibo{[[Cited already..]] They use the width of the range to indicate the  robustness of the optimal plan. This work can be categorized into PQO, but they only interested in the optimality range of the optimal plan. However, if the cardinality estimation can not be trust, then the real robust plan may not be the optimal one originally. In this work, when select the plan for the query, they do not consider the uncertainty of cardinality. While, during execution, their strategy is, if they observe the cardinality of the specific predicate breaks the range, they will switch to another plan.}


==> 10-revision-letter.tex <==
% \documentclass[sigconf,dvipsnames]{acmart}
% \usepackage{graphicx}
% \usepackage{pifont}
% \usepackage{xr}
% % \usetikzlibrary{trees,topaths,calc,shapes.geometric,arrows.meta,positioning,intersections,fit,decorations.pathreplacing}

% \makeatletter
% \newcommand*{\addFileDependency}[1]{
%   \typeout{(#1)}
%   \@addtofilelist{#1}
%   \IfFileExists{#1}{}{\typeout{No file #1.}}
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{
%     \externaldocument{#1}
%     \addFileDependency{#1.tex}
%     \addFileDependency{#1.aux}
% }
% % %%% END HELPER CODE

% % % put all the external documents here!
% \myexternaldocument{main}

% % \lstset{aboveskip=1pt,belowskip=1pt}

% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%



% \newcommand{\reva}[1]{{\leavevmode\color{blue}{#1}}}
% \newcommand{\revb}[1]{{\leavevmode\color{Magenta}{#1}}}
% \newcommand{\revc}[1]{{\leavevmode\color{red}{#1}}}
% \newcommand{\common}[1]{{\leavevmode\color{Plum}{#1}}}


% table cell with breakline
% \newcommand{\specialcell}[2][c]{%
%   \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

% % Definition of circles
% \def\firstcircle{(0,0) circle (1.5cm)}
% \def\secondcircle{(0:0) circle (1.2cm)}
% \def\thirdcircle{(0:0) circle (.9cm)}

% \colorlet{circle edge}{blue!50}
% \colorlet{circle area}{blue!20}

% \tikzset{filled/.style={fill=circle area, draw=circle edge, thick},
%     outline/.style={draw=circle edge, thick}}


% \tikzset{
%     every node/.style={font=\sffamily\small},
%     main node/.style={thick,circle,draw,font=\sffamily\Large}
% }



% \lstset{
%   basicstyle=\ttfamily,
%   breaklines=true,
%   mathescape
% }
 


%\newcommand{\reva}[1]{{\leavevmode\color{BlueViolet}{#1}}}
%\newcommand{\reva}[1]{{\leavevmode\color{ForestGreen}{#1}}}
%\newcommand{\revb}[1]{{\leavevmode\color{Magenta}{#1}}}
%\newcommand{\revc}[1]{{\leavevmode\color{red}{#1}}}
%\newcommand{\common}[1]{{\leavevmode\color{Plum}{#1}}}

% \newcommand{\attrset}{\mathbb{A}}


% \newcommand{\dl}{~{:}{-}~}
% \renewcommand{\vec}[1]{{\mathbf{#1}}}

% \usepackage{cleveref}
% \usepackage[algo2e,linesnumbered,ruled,vlined]{algorithm2e}
% \input{macros}


% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{note}[theorem]{Note}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem*{lemma*}{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}

%%
%% \BibTeX command to typeset BibTeX logo in the docs
% \AtBeginDocument{%
%   \providecommand\BibTeX{{%
%     \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}



% \makeatletter
%   \let\@copyrightspace\relax
%   \makeatother

% \settopmatter{printacmref=false}
% \setcopyright{none}
% \renewcommand\footnotetextcopyrightpermission[1]{}
% \pagestyle{plain}

% \begin{document}

% \settopmatter{printacmref=false}
% \setcopyright{none}
% \renewcommand\footnotetextcopyrightpermission[1]{}
% \pagestyle{plain}
% \pagenumbering{gobble}

% \title{Response Document for Qr-Hint: Actionable Hints Towards Correcting Wrong SQL Queries}


% \renewcommand{\shortauthors}{}



% \maketitle

\section*{Revision Letter: Main Changes}
 % \ag{Three high level comments about the letter: (1) always refer to the most specific updated part (e.g., don't give section refs, give paragraphs in sections), (2) In the main changes, try to group changes from the same section, (3) in the response to a comment, remove the author feedback comment and give the `essence' of the change you've made in the paper (it's ok to copy some of the text that you've added/changed).}

We thank the reviewers for giving us the opportunity to revise the paper, which helped us improve it significantly.
%
Before detailing our responses to comments from each reviewer, here are the most prominent changes:
\begin{itemize}
\item The experiment section (\Cref{sec:expr}) is completely rewritten.
We re-ran all experiments to address concerns such as the PostgreSQL version and test/train separation.
Two more benchmarks, DSB and STATS(-CEB), have been added per suggestions.
We re-positioned the evaluation metric per suggestion.
There is also an in-depth discussion of the optimization overhead, and how the PGO setting addresses it.
Since we cannot possibly fit everything within the page limit,
we summarized the results on DSB and STATS and pointed to the full version of this paper~\cite{fullversion} for details.
\item To clarify error profiling, we have extended \Cref{sec:erorr}
and added one more experiment baseline in \Cref{fig:ablation} in \Cref{sec:expr} to explain how we handle dependency among selectivities.
\item To help with positioning, we have rewritten a significant portion of the introduction; related work has also been extended with missing references.
\end{itemize}
It was impossible to add all new contents to the paper without exceeding the page limit.
Therefore, some old contents have also been moved to~\cite{fullversion}.

Updates made in response to specific comments are color-coded in the paper as follows:
\begin{itemize}
% \itemsep0em
\item \common{Changes in response to multiple reviewers and the meta reviewer are in Purple.}
\item \common{Other generic improvements are also in Purple.}
\item \reva{Reviewer \#3 in Blue.}
\item \revb{Reviewer \#4 in Magenta.}
\item \revc{Reviewer \#5 in Red.} 
\end{itemize}
(Other changes and improvements not addressing any specific comments are not color-coded.)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Meta-Review}

\paragraph{\textbf{M1}} \emph{Kindly justify the conceptual model more rigorously. Why are the 2 questions mentioned on page 1 comprehensive with respect to robust query optimization? Why are the assumptions made in the paper - expressed in the "answers", reasonable? What application-level evidence do you have? Also answer to Reviewer 3 Q14 - R1 and R2, Reviewer 4 Q7 - W1, Reviewer 5 Q7 - W1.}

\common{%
Thank you for the suggestion!
The two questions/answers we posed was not intended to be comprehensive, and in retrospect, they probably have weakened the positioning of our work.
We have now completely rewritten a significant portion of \Cref{sec:introduction} to present a more comprehensive argument for our approach.
Please also refer to our more detailed responses below to specific review comments related to this comment.}

\paragraph{\textbf{M2}} \emph{There has been significant developments in Parametric Query Optimization in recent years. Please place your model in perspective to those work (as some of that work also strives to reduce runtime error), Likewise, there has been recent work studying impact of cardinality estimation (including uneven impact of cardinality errors on plan choice). You must explain how your work leverages developments in these two topics. If your work ignores these developments, please give a rigorous justification.}

\common{%
We are not exactly sure which specific reviewer comments and what additional references this comment refers to.
In addition to addressing related work that the reviewers mentioned (some of which are related to PQO and study of the impact of cardinality estimation),
we have added another particularly relevant piece of recent work~\cite{lee2023analyzing} on understanding the impact of cardinality estimation on plan choice.
If we are still missing any related work, we will be happy to address them!}

\paragraph{\textbf{M3}} \emph{You must provide more complete details of Error Profiling, including the degree to which such profiling is needed, the impact of sampling from this space. Overall, many details are overlooked leaving us little understanding of this component. Specifically, also address Reviewer 4 Q7 - W2, Reviewer 4 Q13 - D4 and D9.}

\common{%
We have add more details on error profiling in \Cref{sec:error} and \Cref{sec:expr}, including an additional experiment.
We do realize now there was a misunderstanding regarding our independence assumption, which should be clarified in the revision.
We also refer to you to more detailed responses below to the relevant reviewer comments.}

\paragraph{\textbf{M4}} \emph{Significantly expand empirical evaluation. This ask is common across reviewers. Please address Reviewer 3 Q14 (R3 – R6) as well as asks in this regard in the reviews by Reviewer 4 and 5.}

\common{%
We have significantly expanded empirical evaluation, including re-running JOB and adding the two new benchmarks suggested.
Consequently, \Cref{sec:expr} was completely rewritten, and various numbers throughout the paper were updated to reflect the new results.
Please see detailed responses below to the relevant reviewer comments.
We hope you will find the revised experiments and discussion a lot more informative!}

\paragraph{\textbf{M5}} \emph{There are presentation issues that reviewers have highlighted. These changes must be done as some of your writing has seeded confusion regarding the model you are proposing. Please take care of any presentation issues (and questions arising from those issues) flagged in any part of the three reviews.}

\common{%
Done. Please see detailed responses below to the relevant reviewer comments.}

\paragraph{\textbf{M6}} \emph{Please address all remaining required changes (Reviewer 4 - Q14, Reviewer 5 - Q14, and Reviewer 6 - Q14) unless covered by the required changes already listed above. In addition, try to address all other aspects flagged in the detailed reviews (responses in Q7 by the reviewers).}

\common{
All done.  Please see detailed responses below to the relevant reviewer comments.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer \#3}

\paragraph{\textbf{Requested in Q14: R3R1/O1/D1}} \textbf{R3R1}. \emph{[O1] Add justification for the proposed metric.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R3O1}. \emph{It seems that the basis of this work is the new metric of robust plan selection. However, the metric needs more justification given that basically almost all prior attempts on new metrics for query optimization fail to be used in practice, even though they are more intuitive than the one proposed by this work.}
    \\\common{We do not advocate for the specific metric in \Cref{eq:penalty}.
    Rather, we argue that there is no one-size-fit-all metric;
    thus, we want a framework that allows a flexible and powerful metric specified by application needs,
    as well as associated methods that are general enough to handle such metrics while still playing nicely with existing database systems
    (we have rewritten a significant portion of the introduction to make this high-level point more clear).
    We chose the metric in \Cref{eq:penalty} such that it illustrates the challenge of supporting a general metric.
    First, it measures the penalty of a plan relative to the would-be optimal plans,
    so it is impossible to independently assess a plan's robustness without understanding where it stands with competing plans.
    Adding a threshold is common in robustness metrics (e.g., \cite{harish2007production, 2018rqo, dutt2014plan, dey2008efficiently}),
    and it also adds some non-linearity --- had we used simple difference or ratio relative to the optimal,
    it would have been possible to solve a simpler and more specialized version of the optimization problem,
    which we do not want since we want to illustrate the generality of our framework.

    Indeed, much previous work, with various robustness metrics, seems to have failed in gaining adoption.
    We believe the issue is not with the particular metric per se.
    Rather, the issue is that they support \emph{one specific} metric
    by developing rather elaborate machinery that require non-trivial modification to the database core (often for good reasons such as efficiency).
    But this specialization hurts their adoption, because they only work for very specific notions of robustness.}

    \item \textbf{R3D1}. \emph{Robust query optimization has been around for a long time, and prior work has proposed alternative objective functions for robust query optimization compared to traditional QO, such as [1] and [2]. Unfortunately, it seems that almost none of these attempts have made their way to real database systems. Given these objective functions are even more intuitive than the proposed metric (i.e., even the most basic form), it needs to provide more justification of why the proposed problem formulation is interesting and relevant, even if it is more general.\\
    1. Brian Babcock, Surajit Chaudhuri: Towards a Robust Query Optimizer: A Principled and Practical Approach. SIGMOD Conference 2005: 119-130\\
    2. Yifan Li, Xiaohui Yu, Nick Koudas, Shu Lin, Calvin Sun, and Chong Chen. 2023. DbET: Execution Time Distribution-based Plan Selection. Proc. ACM Manag. Data 1, 1, Article 31 (May 2023), 26 pages. https://doi.org/10.1145/3588711}
    \\\reva{We have given a more general response above, but here are our responses specifically on these two references.
    Both [1] and [2] assume we can derive a distribution of plan cost capturing its uncertainty;
    then, they look for the plan whose 80-percentile cost (or some other prescribed threshold) is the lowest.
    This is a perfectly fine metric, but a specific one that does not fit all application needs.
    It is also not the most challenging metric to optimize for, because it is not penalty-based and can be assessed independently from competing plans.

    [1] has been around for a while and one could ask why it has not been adopted.
    Again, we do not think it is due to the metric per se, but rather,
    it requires modifying the optimizer (to be distribution-aware) and execution engine (to obtain cardinality distributions with sampling-based methods at runtime), which might have been too much ask for to support one specific metric.

    [2] is new, so we would rather not predict whether it will stick, but an important distinction from our work
    is that it uses a deep-learning approach to directly predict the cost distribution for a plan.
    Aside from requiring lots of training data, this approach is opaque.
    Our approach has the advantage of being interpretable ---
    our sensitive dimensions can be explained to users and can be used to reduce dimensionality when solving the subsequent optimization problems.}
\end{itemize}

\paragraph{\textbf{Requested in Q14: R3R2/O2/D2}} \textbf{R3R2}. \emph{[O3]\footnote{\reva{The review tagged this item as O3, but from the context it seems to be O2.}} Fix the positioning of this work, or describe how to use the proposed technique for query optimization and evaluate properly.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R3O2}. \emph{The positioning of this work is a bit misleading. From the evaluation setup, this work seems to be more like robust plan selection instead of robust query optimization. It is not clear how the proposed technique can be integrated into the query optimization process with low overhead given the large number of subplans in the search space.}
    \item \textbf{R3D2}. \emph{If I understand correctly, the main technical section is about quantifying the penalty of query plans and selecting the most robust one among them. It is not clear if the focus of this work is really “query optimization” or simply “plan selection”. If it is the former, it needs more elaboration on how to control of the overhead of the query optimization given the large number of subplans in the search space; otherwise, the paper needs to be positioned properly.}
\end{itemize}
\reva{%
Robustness metric for plan selection is indeed a big part of our contribution,
but we would like to emphasize that we do want to offer a practical end-to-end solution that plays nicely with existing database systems.
The latter desideratum limits us to making \Opt\ and \Cost\ calls to existing optimizers without fiddling with internals,
and to using traditional plans as opposed ones that can adapt at runtime.
Perhaps this is what gives our work a ``plan selection'' feel.
We hope the revised introduction address this positioning issue, along with a completely rewritten evaluation section (see also our response to R3R4/D3 below).

We do care about the overhead, so we have added a lot more details in \Cref{sec:expr} to quantify the various overheads and provide a cost-benefit analysis.
Briefly, robust optimization runs on the order of minutes,
so it is not a good deal for completely ad hoc queries unless they run very long on massive datasets
(fortunately our optimization time does not depend on data volume).
However, the calculation changes in our favor in the PQO setting where we can amortize the upfront one-time optimization overhead over many instances of the same query template.
For production databases that are frequently queried with popular query templates, the break-even point can be reached pretty soon.
We also quantify the runtime optimization overhead of our PQO (which involves KL-divergence testing not in standard PQO),
and confirm that it is lower than traditional optimization.}

\paragraph{\textbf{Requested in Q14: R3R3/D5}} \textbf{R3R3}. \emph{[D5] Evaluate on more workloads, including TPC-DS/DSB and STATS-WEB.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R3D5}. \emph{The evaluation needs to be performed on additional workloads, including TPC-DS, STATS-CEB [5], and DSB [6].\\
    5. Yuxing Han, Ziniu Wu, Peizhi Wu, Rong Zhu, Jingyi Yang, Liang Wei Tan, Kai Zeng, Gao Cong, Yanzhao Qin, Andreas Pfadler, et al. 2021. Cardinality Estimation in DBMS: A Comprehensive Benchmark Evaluation. VLDB Endowment (2021).\\
    6. Ding, Bailu, et al. "DSB: A decision support benchmark for workload-driven and traditional database systems." Proceedings of the VLDB Endowment 14.13 (2021): 3376-3388.}
\end{itemize}
\reva{Thanks for the suggestion!}
\common{DSB (which subsumes TPC-DS) is especially a great fit because it fully specifies its query workload distribution, saving us the trouble to define one ourselves.}
\reva{STATS(-CEB), too, with some really expensive queries, also improved our understanding of the problem.
We have significantly expand our experiments to include both of these benchmarks, though it was a struggle to figure out how make everything fit within 12 pages.}

\paragraph{\textbf{Requested in Q14: R3R4/D3}} \textbf{R3R4}. \emph{[D3] Compare to [3] and [4] for end-to-end query performance and the penalty metric (on the selected plan).}
\begin{itemize}[leftmargin=*]
    \item \textbf{R3D3}. \emph{It seems that the evaluation metric of the proposed technique is in fact the query execution time instead of the penalty function (i.e., the objective function for selecting the plan). While the end-to-end query performance is of course interesting, it unfortunately also positions this work into a crowded space. Given the proposed technique also needs data collection and some kind of training, it is meaningful to compare this work with recent work using learned cost estimates such as [3] and [4]. However, it seems the performance of the proposed technique is not very attractive in terms of end-to-end query performance. It will be more interesting to compare this work with prior work on learned cardinalities for both the end-to-end query performance as well as the penalty metric.\\
    3. Wu, Ziniu, et al. "FactorJoin: a new cardinality estimation framework for join queries." Proceedings of the ACM on Management of Data 1.1 (2023): 1-27.\\
    4. Gu, Rong, et al. "ShadowAQP: Efficient Approximate Group-by and Join Query via Attribute-Oriented Sample Size Allocation and Data Generation." Proceedings of the VLDB Endowment 16.13 (2023): 4216-4229.}
    \\\reva{This is a great point, related to the R3D2 above.
    Thank to this comment, we realize our mistake of first presenting execution time results on a single database instance, without proper positioning,
    gives the wrong impression that it is what we care most.
    It is not our intention at all; we ultimately care about robustness, which can only be measured over many possibilities instead of a single database instance.
    Indeed, most of our experiments after the first aimed at measuring robustness better.
    We have completely rewritten \Cref{sec:expr}, reworked its flow, and re-positioned this first experiments so there is no misunderstanding.

    Regarding the suggestion to compare with [3] and [4]: perhaps with the above clarification and repositioning,
    it is already already apparent that they are orthogonal contributions not suitable for direct comparison.
    For [3], we are not targeting improving cardinality estimation itself.
    \OurSys\ is designed to provided add benefit of robustness when prediction misfires.
    As FacorJoin [3] does not provide its own error estimates, we can collect error profile as we do for PostgreSQL,
    but the rest of the framework remains unchanged.
    Perhaps a more appropriate comparison would be FactorJoin with or without \OurSys,
    but we feel it is out of the current scope of our paper (not mention that are many other cardinality estimation papers to compare with too).
    As for [4], it targets a very different problem of approximate query processing,
    an alternative approach to scalability using approximate query answers;
    \OurSys\ tries to improve traditional, exact query processing.}
\end{itemize}

\paragraph{\textbf{Requested in Q14: R3R5/D4}} \textbf{R3R5}. \emph{[D4] Fix the evaluation setup.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R3D4}. \emph{The setup of the evaluation for single query performance is strange as the error profile includes the errors collected from all queries. It is almost analogous to use the same dataset for both training and testing. It will be more interesting to split the data sets into the ones used for error profiling and the ones for the actual evaluation.}
\end{itemize}

\common{In the process of rerunning all experiments on JOB on the lastest version of PostgreSQL (see also R4D6) and adding more on DSB and STATS, we followed this suggestion and took care in ensuring that there is always a clear separation between training and testing.
First, for JOB, the benchmark specifies several instances for each query template, labeled further by (a), (b), etc.; we used the 33 instances labeled (a) for evaluation and the remaining 80 with other labels for constructing the error profile and collecting the distribution of query literals (see the beginning of \Cref{sec:expr}).
For DSB, where the benchmark specifies the synthetic query distribution, we used different random seeds to generate queries for testing and for constructing the error profile (see our full version  \Cref{app:expr}).
For STATS, we randomly chose 26 out of the 146 benchmark queries, with the constraint that they cover the entire range in terms of query complexity from 3- to 7-table joins, and constructed 22 query templates for evaluation based on the chosen queries; the remaining 120 queries were used for constructing the error profile and collecting the distribution of query literals (see  \Cref{app:expr}).}

\paragraph{\textbf{Requested in Q14: R3R6/D6--8}} \textbf{R3R6}. \emph{[D6-D8] Report overhead of plan generation and selection. Clarify D7 and D8.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R3D6}. \emph{Does the query end-to-end performance include the overhead of generating plans and selecting a robust plan? If not, please report the overhead in the evaluation.}
    \\\common{We have now provided details on overhead in \Cref{sec:expr} and \Cref{app:expr} for all three benchmarks, including an analysis of when the PQO setting is expected to reach the break-even point to overcome the initial overhead for PQO (see also our response to R3R2 earlier).}
    \item \textbf{R3D7}. \emph{It seems that Sobol’s method almost always outperforms Morris method, is there any reason to use Morris at all?}
    \\\reva{It is true that Sobol's picks better sensitive dimensions than Morris.
    However, Morris is also very popular in practice because it is computationally less expensive.
    Thus, we want to evaluate both in our application setting.
    That said, we moved details on Morris from \Cref{sec:sensitivity} to~\cite{fullversion} in order to save space.}
    \item \textbf{R3D8}. \emph{The evaluation section says “To obtain the actual execution time of each plan, we executed the query with this plan as hint 101 times and recorded the median result.” Why 101 times? Is this a typo?}
    \\\reva{It is not a typo; we indeed ran each plan 101 times to get the median result.
    We did so to improve repeatability because measured running times often exhibited noise.
    In retrospect, 101 repetitions per plan were an overkill.
    In this revision, for JOB and DSB, we used 11 repetitions in PQO experiments and 101 repetitions in other experiments;
    for STATS, we used 5 repetition in all experiments because some STATS queries took more than 20 minutes to run.
    We added a remark at the beginning of \Cref{sec:expr}.}
\end{itemize}

\paragraph{\textbf{R3O3}} \emph{While the problem formulation and the sensitivity analysis are kind of principled, the construction of the input to these approaches is very heuristic. It is not clear how principled the end-to-end result is. The same applies to the use of KL divergence for parametrized queries.}

\reva{Regarding the concern that ``construction of the input'' being heuristic,
we interpret it to mean one of the following issues.
First is the construction of error profiles, and in particular the concern that we appear to be assuming independence of errors in different selectivities.
We clarify the latter in our detailed response to R4D5.
In short, our approach is able to capture some dependencies (up to among one join and two local selections that appear together in a querylet),
but we have to resort to the tried-and-true technique of factorization to tame the cost of modeling the full joint error distribution.
Overall, we do not claim that we have the best solution for constructing error profiles;
our goal was to demonstrate a simple and effective method that one can always fall back to,
but it certainly can be replaced by more sophisticated methods or aided by other information that might be available.

The second source of your concern may be the space of the robust plans, which we obtain by sampling the optimal plans at different selectivity settings.
While this approach seems to have worked well on the benchmarks we tested,
we fully recognize that it is only a heuristic,
and we discuss the challenge of ensuring optimal robustness as future work in \Cref{sec:conclude};
that will likely require close interaction with an optimizer's inner workings, which we have avoided so far.

Regarding the concern about KL divergence, we are not sure where it stemmed from.
Recall from \Cref{footnote:kl} that our test compares $f(\sels | \hat\sels)$ and $f(\sels | \hat\sels')$,
which are distributions of \emph{true} selectivities.
If these distributions are indistinguishable,
the two queries would be indistinguishable from the perspective of selecting robust plans by problem definition.
Of course, there can still be the concern about the error profiles used to derive $f(\sels | \hat\sels)$ and $f(\sels | \hat\sels')$ in the first place,
but that is an orthogonal concern addressed earlier.}

\paragraph{\textbf{R3O4/D3--8}} \emph{The proposed technique does not seem to be very attractive in the evaluation given the evaluation metric. Also, the evaluation needs to be enhanced with more realistic setup and additional workloads.}

\reva{We addressed this issue in the contexts of R3R4/D3, R3R5/D4, R3R3/D5, and R3R6/D6--8; see above for detailed responses.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer \#4}

\paragraph{\textbf{Requested in Q14: R4W2/D4,5}} \textbf{R4W2}. \emph{The collection of the error profiles is scarce in important details and makes assumptions that are not clearly stated.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R4D4}. \emph{"we use the median error as the low-high cutoff in this paper" --> How do you obtain the median error?}
    \\\revb{Recall that we collect all observed errors in a given selectivity in an error profile;
    we simply pick the median among the observed errors.
    We have clarified this in \Cref{sec:error}.}
    \item \textbf{R4D5}. \emph{"Second, the independence assumption made by many traditional optimizers is often blamed for throwing off cardinality estimates; hence, we need to go further than profiling each selection predicate and join predicate in isolation, so we can account for the effect of their interactions on estimation errors." and "Finally, to put together the error distribution in ŝ in the full -dimensional selectivity space, we assume independence of errors across dimensions." --> These two statements seem to be contradictory.}
    \\\common{Indeed, our submission did not do a good job explaining what we did to capture dependency in error profiling
    (our overloading the term ``dimension'' probably causes your confusion --- sorry!).
    We have now cleaned up the sentence leading to \Cref{eq:sel-pdf} in \Cref{sec:error} and added a discussion paragraph after it;
    together with the complete example we added in response to R4D3, we hope the explanation is more clear.
    In brief, besides single-table querylets,
    we introduced error profiles of two-table querylets to capture dependencies between a join and local selection conditions on the joining tables;
    for a binary join that never has any local selection conditions attached, we further profile three-table querylets involving this binary join --- intuitively, to capture the dependency between this join and its surrounding context.
    In reality, we cannot afford to track the full joint distribution of all selectivities,
    so we have resorted to the idea of factorizing the full distribution ($f$) into more manageable factors ($g_i$'s),
    some of which (namely, those derived from two- and three-table querylets) do capture dependencies.
    Multiplying factors does \emph{not} mean assuming independence among the selectivities they cover.
    To show the practical benefit of this approach of capturing dependencies,
    we also added a new experiment in \Cref{sec:expr} comparing our approach with a baseline where join and selection selectivities are profiled in isolation.}
\end{itemize}

\paragraph{\textbf{Requested in Q14: R4W3/D1,2}} \textbf{R4W3}. \emph{The writing requires some significant work. Also, if an extended version exists, it should be correctly referenced.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R4D1}. \emph{"see the extended version of this paper [?] for details" --> There is no reference to an extended version.}
    \\\revb{Fixed.}
    \item \textbf{R4D2}. \emph{"recall from ?? that PostgreSQL invokes more than 13,000 cardinality estimates" --> What is "??"?}
    \\\revb{Fixed.}
    \item \textbf{R4D3}. \emph{"For example, for Q17, we would arrive at d = 12." --> It would help if you enumerate the 12 dimensions. In fact, it would be even better if you illustrate the entire process in Section 3 based on the example query Q17.}
    \\\revb{We have now enumerated all 12 dimensions and explained how they were derived; see \Cref{sec:error}.}
    \item \textbf{R4D7}. \emph{The captions in many figures are very hard to read, e.g., Figure 2, 5, 6, and 7.}
    \\\revb{We have enlarged the font size in these figures (their numbers have shifted in the revision).}
\end{itemize}

\paragraph{\textbf{Requested in Q14: R4D6}} \emph{"PostgreSQL V12.5 was used as the optimizer for end-to-end analyses." --> Why do you use V12.5 when there is already a V16.2 available? The query optimizer changed quite a bit over the latest releases.}

\revb{We have upgraded PostgreSQL to its latest version (16.2) and integrated our system to interact with the newest optimizer.
We have rerun all old experiments on the new setup and updated the numbers in \Cref{sec:expr} and throughout the paper;
there were some differences but they were minor.}

\paragraph{\textbf{Requested in Q14: R4D8}} \emph{"PARQO believes that "what matters" depends on the application scenario, and that many scenarios require us to define robustness in more nuanced ways, such as in terms of a penalty relative to the optimal plan had we known true selectivities." --> In query optimization, this notion is called P-error. The authors do not seem to be aware of it.}

\revb{We are aware of~\cite{han2021cardinality} (which we cited earlier because we followed its approach of instrumenting PostgreSQL) and the notion of P-error it introduced.
We have now added a reference to P-error when discussing our metric; see \Cref{footnote:other-penalties}.
P-error is a fine metric but there is an important difference between P-error and our choice in \Cref{eq:penalty}:
unlike our choice, log-P-error is only ``pseudo-dependent'' on the optimal plan costs,
which leads to a simpler and more specialized optimization problem, not suitable as an example to illustrate the generality of our framework.
(Fine print: note that we consider log-P-error instead of P-error here --- since P-error is a ratio, it may be undesirable to use its expectation, or arithmetic mean, directly as an objective.)}

\paragraph{\textbf{Requested in Q14: R4D9}} \emph{"selected sensitive dimensions correspond to selection/join condition combinations in the query, which are interpretable and actionable --- for example, a user may investigate a sensitive dimension and improve its accuracy in order to obtain a better plan." --> While I agree with the interpretable part, I am not so convinced about the actionable part. What methods are proposed to improve only a subset of estimates? How do you quantify the impact on the other estimates?}

\revb{Many database systems (e.g. PostgreSQL, SQL Server) allow selective refresh of specific statistics objects down to columns,
so one could target those relevant to the sensitive dimension.
Indeed, doing so may change other cardinality estimates besides the sensitive dimension and may lead to some other surprise, but it is not a crippling issue as it can be observed and overridden by manually injecting revised estimates if desired.
More generally, one could also employ sampling-based methods for estimating the size of the subquery corresponding to the sensitive dimension,
and then inject the new estimate.
To explain, we have added a parenthesized remark in \Cref{sec:introduction} as well as \Cref{footnote:get-true-sel} in \Cref{sec:expr}.}

\paragraph{\textbf{R4W1}} \emph{I am not convinced that the proposed solution is actionable because of its interaction with the other complex parts of the query optimizer.}

\revb{In contrast to much of the previous work on robust query optimization,
we have designed \OurSys\ to require as little modification to existing query optimizers as possible.
The only requirement is that the database allows $\Opt$ and $\Cost$ calls and the execution of a given plan, without exposing the inner workings of its optimizer.
For PostgreSQL, we were able to do so with the \texttt{pg\_hint\_plan} extension (for specifying a particular execution plan)
and with slight modifications to the optimizer code (for injecting specific cardinality estimates).
While the latter may sound messy, the modifications (documented in our GitHub repository) were actually straightforward
and did not change how the PostgreSQL optimizer works otherwise.
It would be relatively straightforward to enable such hooks in other database systems if the vendors so choose.
Assuming these above hooks, the whole framework can be realized a middleware layered on top of a database system.
Error profiling, identifying sensitive dimensions, finding robust plans, plan caching, and parametric query optimization can all be done in this layer without modifying the underlying database systems and in a way transparent to the applications.

That said, a tighter integration with the database internals would support a larger search space for robust plans (as discussed in \Cref{sec:conclude})
as well as more efficient error profiling via runtime monitoring;
these would be nice-to-have features for future work, but they are not required for \OurSys, which already delivers tangible benefits without complex interactions with the underlying optimizer.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{Reviewer \#5}

\paragraph{\textbf{Requested in Q14: R5W1/D1}} \textbf{R5W1}. \emph{Some design choices could be justified or motivated more carefully, see the detailed comments D1.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R4D1}. \emph{The motivation states that the paper provides answers to two questions. The motivation and the choice of answers would be more convincing if they were justified with data, e.g. based on issues in real-world scenarios. For example, it might be debatable, if "just" focusing on a known workload is sufficient (vs. gracefully handling also unknown workload).}
\end{itemize}
\common{Thank you for this comment --- it made us we realize that we failed to provide a more comprehensive motivation for our work in our initial submission.
As a result, we have completely rewritten this portion of the introduction, which hopefully provides a better justification (and beyond the two question/answer pairs).
As to the specific question about handling unknown workload,
we have added \Cref{footnote:cold-start} in \Cref{sec:error} to handle this ``cold-start'' problem.
Perhaps you are alluding also to the challenge of coping with dynamic workloads,
which we discuss as future work at the very end in \Cref{sec:conclude} --- it is a hard problem in general.}

\paragraph{\textbf{Requested in Q14: R5W2/D2}} \textbf{R5W2}. \emph{While JOB is a reasonable benchmark for evaluation, limiting the analysis to only selected queries is a bit narrow. I would recommend to have also an aggregated experiment for all JOB queries. Also the DSB benchmark provides a great workload for this topic.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R4D2}. \emph{D2: I would appreciate also a broader evaluation demonstrating the robustness of the method beyond selected queries of JOB, e.g. covering all JOB queries. DSB (https://vldbarc.org/pvldb/vol14/p3376-ding.pdf) would also be a good candidate for evaluating parametric queries or evolving databases.}
\end{itemize}
\revc{Regarding queries in JOB, we have in fact experimented with all of them.
JOB divides all its 113 queries into 33 templates; for each template, we reserved one query for testing and the others for error profiling, per suggestion of R3R5/D4.
Thus, every one of the 33 templates is represented in our results.}

\common{Regarding DSB, thank you for this great suggestion!
It is indeed a good fit for our setting since it specifies the query workload explicitly.
We have added experiments on DSB (with details in \Cref{app:expr}); see also our response to R3R3/D5.}

\paragraph{\textbf{Requested in Q14: R5W3/D10}} \textbf{R5W3}. \emph{There are a number of presentation issues, e.g. typos, that shall be fixed.}
\begin{itemize}[leftmargin=*]
    \item \textbf{R4D10}. \emph{Please address the following presentation issues: ...}
\end{itemize}
\revc{Fixed.}

\paragraph{\textbf{R5D3}} \emph{I agree that the panelty function should be pluggable. For the function presented in Eqn (1) it is, e.g., debatable why the tolerance should be proportional to the optimal cost? For example for "cheap plans" we might be more tolerant. Or the execution frequency determines the tolerance. Please justify why the chosen tolerance and penalty function is reasonable.}

\common{%
This is a great point.
We picked the relative threshold of 120\% because it has been very a popular choice in robust query optimization literature~\cite{harish2007production, 2018rqo, dutt2014plan, dey2008efficiently}.
However, idea of setting absolute instead of relative thresholds for fast queries makes a lot of sense,
so is the idea of using the execution frequency in setting tolerance.
We thought about changing our default metric,
but then realized that it would become very inconsistent with at least one method (WBM) that we compare with directly,
and it require additional parameters whose particular settings would be hard to justify too.
Also, we note that we are not advocating for the specific metric in \Cref{eq:penalty}.
Rather, we argue that since there is no one-size-fit-all metric, we need it to be pluggable.
We chose the metric in \Cref{eq:penalty} because it has properties that illustrate the genearlity of our framework and methods.
Please see also our detailed response to R3R1/O1/D1 on this point.}

\paragraph{\textbf{R5D4}} \emph{Note, the complexity of a query can also be derived from the query graph and considered shapes of join trees. But counting the calls to cost is at least an indication of the examined size of the search space.}

\revc{Agreed.
We assume you are referring to the example about Q29 in \cref{sec:introduction};
we made it more precise by adding the number of self-joins in this query.}

\paragraph{\textbf{R5D5}} \emph{Note that the idea of storing (sub-)plans was considered before. For example, Microsoft has a QueryStore
(https://learn.microsoft.com/en-us/sql/relational-databases/performance/monitoring-performance-by-using-the-query-store?view=sql-server-ver16)
that was also used in academic papers by Microsoft.}
\\\revc{Thanks for the suggestion.
We have cited this technical blog in \cref{sec:related} and categorized it as an online-based method in PQO.}

\paragraph{\textbf{R5D6}} \emph{Note that the query profiles based on querylets can also be pruned. For example, filters over unique (sets of) columns likely do not need to be profiled. Please also elaborate on the memory consumption when collecting of the query profiles, i.e. what if it uses exceeding amounts of memory? how are selectivities on filters with many conditions addressed, e.g. range predicates over columns with many distinct values or string pattern matching?}

\revc{This is a great suggestion;
indeed, with database constraints, a good selectivity estimator should produce no error for certain selection and join conditions.
We did not explore such opportunities fully (other than skipping some very obvious cases where only the base table cardinalities were needed),
because we simply wanted to present a simple method that one can always fall back to without assuming we know how smart the estimators are.

We have not observed any memory issues at all when profiling errors for all three benchmarks,
partly because we have rather coarse models
that only differentiate low vs.\ high initial estimates
and do not differentiate different forms of predicates such as range vs.\ pattern as you mentioned.
For each of the three benchmarks we tested,
our overall model size was under 15KB,
and the total memory taken by statistics during error profiling was under 200KB.
Higher accuracy can certainly be achieved with higher-resolution models and additional profiling effort,
but for this work, our goal is to demonstrate a simple yet effective enough method;
more sophisticated methods can be plugged into our framework easily.}

\paragraph{\textbf{R5D7}} \emph{Section 3 states the assumption that errors are independent across dimensions. This may not be the case in the presence of correlation. Please elaborate on the impact of this assumption.}

\common{We in fact do \emph{not} assume that errors are independent across dimensions ---
our submission did not do a good job explaining what we did to capture dependency in error profiling.
We have now cleaned up \Cref{sec:error} and added a discussion paragraph after \Cref{eq:sel-pdf};
together with the complete example we added in response to R4D3, we hope the explanation is more clear.
We have also extended one of our experiments to how our approach beats one that assumes independence.
Please see our more detailed response to R4W2/D4,5.}

\paragraph{\textbf{R5D8}} \emph{Related to the discussion of parameterized queries, please check https://dl.acm.org/doi/10.1145/3183713.3183742, which computes optimality ranges for queries. These express for which range of selectivities a plan remains optimal. The distance to the boundary of the range can be used as an indicator of plan robustness, but they can also be used to select alternative plans for parameterized queries. Plan diagrams and its successors follow a similar approach.}

\revc{%
Thank you for this pointer.
The range indicator as robustness can be seen in our framework as a special case of a 0-1 penalty function with uniform error assumption.
Indeed it is relevant to PQO and we have discussed it in related work.
Their runtime adaption strategy requires hooks into the underlying database systems that \OurSys\ does not assume, however.}

\paragraph{\textbf{R5D9}} \emph{In the experiments in Fig 5 and 6 it would also be interesting to compare against the plan with the lowest cost (i.e. also disregarding bad choices of the Postgres optimizer).}

\revc{%
PostgreSQL's \Opt\ may not return the optimal plan even if we inject all correct cardinality estimates,
and there is unfortunately no convenient way of finding the best plan that actually delivers the fastest running time
(or even just the lowest estimated cost, for complex enough queries where the search space would be heuristicly pruned).
It will require exhaustively tuning every single query instance in our experiments,
and the effort would be prohibitive.
For the purpose of this experiment (note that figure numbering has changed in the revision),
which is to demonstrate robustness improvement over traditional plan on previously unseen instances,
we hope that by giving PostgreSQL the benefit of seeing refreshed statistics, which \OurSys\ does not have access to,
its plan will provide a reasonable reference point.}

% \end{document}


==> 11-shepherding-letter.tex <==
\section*{Revision Letter to Shepherd}
All updates we made in this revision are highlighted in red color.

\paragraph{\textbf{R1}} \emph{Provide motivating examples on why the proposed framework holds a unique promise of adoption despite failures of many previous attempts at robust query processing.}

\shep{Thank you for the suggestion.
We have rewritten parts of \Cref{sec:introduction} to highlight the specific challenges we addressed
in order to make our proposed framework better positioned in terms of adoption.
We hope that, with the additional changes we made in response to R2 below, the paper is now better motivated than before.}

\paragraph{\textbf{R2}} \emph{Related to R1, the rationale for the framework needs to be strengthened by providing several (at least more than one) practical penalty metrics.}

\shep{Per suggestion, we have added more alternative practical penalty definitions,
how various notions of robustness previously introduced can be encoded in our framework,
as well as how to extend our framework to handle even more sophisticated notions.
We were hoping to add these to~\Cref{sec:framework},
but discussing them properly requires a lot of space, which might be distracting to the reader.
Hence, we have added a summary to~\Cref{sec:framework} and all details to~\Cref{app:alt-robust} (which will be included in the full version).}

\paragraph{\textbf{R3}} \emph{Consider revising how the paper is positioned. I strongly recommend softening the claim that the paper contributes a query optimization technique (e.g., used for plan selection instead of query optimization) given its high overhead.}

\shep{We agree that robust query optimization is a broader topic,
and robust plan selection is the specific task we are focusing on in this paper.
Following your recommendation, we have changed our paper title to ``PARQO: Penalty-Aware Robust Plan Selection in Query Optimization''
and highlighted plan selection in PARQO.}

\paragraph{\textbf{D1 - D12}} \emph{Other minor issues}

\shep{We have addressed all the other minor issues in our last submission. Thanks again for the careful suggestions from all the reviewers.

We also made other (minor) improvements to writing throughout the paper,
which we did not highlight because they were not specific to any shepherding requests.}

==> 6-expr-old.tex <==
To construct $f(\sels | \hat\sels)$ for a given query workload, we narrow our focus to querylets related solely to all 1-table and 2-table querylets, plus additional 3-table querylets as discussed in Section \ref{sec:error}. In real-world scenarios, we should learn from historical executed querylets in the workload. 
\common{To emulate real-world conditions in our experiments, we split the queries into a training set and a testing set, assuming prior knowledge of the training set to profile errors and then evaluating our method on the testing set.}\footnote{\common{The workload of JOB contains several instances for each query template. 33 instances labeled "(a)" are used for actual evaluation, while all other 80 instances are used to collect possible predicate literals and construct error distributions. }}
Then, for each specific querylet, we build a template that involves the exact table(s) in this querylet, apply the collected predicate literals as conditions accordingly to the table(s), and simulate a workload. 
% We execute the simulated workload to obtain true errors. Specifically, for 1-table querylets\footnote{}, e.g. L($k$), we create a template that only involves $k$ and apply all possible selection conditions. Similarly, for 2-table querylets\footnote{}, e.g. L($mc$) join L($cn$), we create the workload by a template that joins $R$ and $S$, adjusting the predicate literals accordingly. The error profile construction for 3-table querylets follows a similar process. 
We collect the \textit{log-relative} errors for $\hat \sels$ by executing the workload and use a Gaussian kernel to estimate the PDF. For each querylet we build two models using the medium error as the low-high cutoff. Some example PDFs can be found in~\cite{fullversion}.

\footnote{\revc{**[[[[We can delete this]]]]**} We apply a zero error on 1-table dimensions lacking local selection or consisting solely of categorical tables with equality predicates, as the optimizer typically operates accurately on these dimensions. For 2-table join, if neither table has local selection, we build PDF by merging the collected error data from all satisfied 3-table querylets. If no 3-table querylet meets the criteria, we simply use a template to join those two without any local selection and collect the error.}

To evaluate the performance of plan selected by \OurSys, we compare the real execution time
with PostgreSQL, WBM\cite{2018rqo} and \textit{recentering} as baselines. 
% We do not wish to dictate a single notion of robustness measurement since it depends on application scenarios. Experiments employing various candidate plan collections, robustness metrics, and $\sensilocal$ will be detailed in the full version. 
As proposed in WBM, non-foreign key joins are considered as sensitive dimensions.
\reva{Across the entire set of 33 queries, \OurSys~ outperforms PostgreSQL's plan in 19 queries, with an average speedup of 4.51x. 
For 9 queries, \OurSys~ and PostgreSQL select plans with similar execution times, and WBM does not choose a faster plan as well. 
In the remaining 5 queries, \OurSys~ selects a plan that performs worse. As shown in Figure \ref{fig:exe-good}, the method based on Sobol's outperforms others in most cases. The most notable improvement in execution time is observed in Q17, where \OurSys's plan takes 620 ms, while PostgreSQL's and WBM's plans take more than 5,000 ms. 
In Q20, \OurSys-Sobol achieves a maximum speedup of 12x compared to PostgreSQL. 
Morris, although not as effective as Sobol's, still surpasses WBM in most cases.} \common{The overall speedup for JOB is 3.23x. For DSB and STATS, the overall speedups are 2.01x and 1.36x, respectively. \common{Detailed experimental results for DSB and STATS can be found in our full version paper.}}

\revc{***[[[[[Maybe delete or short this for space. TODO]]]]]***}Among all queries, WBM's plan performs closely to PostgreSQL. This is attributed to WBM's strategy of focusing on near-optimal candidates only (it filters out any plan with significantly higher estimated costs, e.g., $\Cost(\plan, \hat \sels) > 1.2 \cdot \optCost(\hat \sels)$). When the original plan is already robust at the given selectivity estimates, WBM selects it by focusing solely on that local point, thus benefiting from this approach. 
PostgreSQL's plan and the near-optimal plan may have a low cost value at the original estimates, but they incur a high penalty due to actual errors. In contrast, a truly robust plan might initially exhibit a higher cost value, yet it ultimately demonstrates a lower expected penalty across the error profiles.
\OurSys~ accounts for the selectivity uncertainties informed by the workload and considers the optimal plans across potential selectivity spaces, penalizing the cost differentials relative to the optimal plan directly. 
For example, in Q17, the default plan costs 4.6k at the original estimates, but has a 60k penalty given actual errors. \OurSys~ identifies the most robust plan, which costs 12.5k at estimates but will not be penalized at actual selectivities. Ultimately, our plan performs 5.6x faster in terms of execution time. 
Our experiments highlight that we should not make decision overlooking the potential errors.

% even when a plan has a high estimated cost, we should not exclude it as a candidate, as they may ultimately prove to be robust, despite being overlooked by the cost model due to the unknown real selectivity at runtime.

We also observe that for several queries, \common{such as Q2, 26, and 30}, the recentered plan already exhibits a speedup. This indicates that our error profiling, despite its simplicity \common{(only 13.8 KB)}, can correct certain biased estimations. However, because of its rather coarse granularity, it is not always effective in driving improvements directly such as cases of \common{Q7, 18, and 20}.
For queries where our robust plan costs similarly or even higher than PostgreSQL's,
we note that this experiment only compares their cost at one particular data point,
with PostgreSQL having the advantage of specifically optimizing for this point while we optimize for robustness against various possible errors.
\revc{****Need huge revision in this paragraph.****}
Indeed, in latter settings such as PQO where we examine costs across many queries,
we see our robust plans still come out on top.
Nonetheless, for queries where \OurSys~ does not perform optimally in Figure \ref{fig:exe-bad}, we provide a breakdown of the reasons.
For instance, Q1 has a sensitive dimension matching $it^\select \join mi\_idx$ with \textit{it.info = `top 250 rank'}.
It happens that our error profile misestimated the error for this particular parameter setting.
Similarly, for querylet $mk \join k^\select$ in Q3, 4, and 6, and $cn^\select \join mc^\select$ in Q15,
the error profiles misestimated errors in these dimensions.
However, when we examine plan performance under the PQO settings, we see our robust plans indeed exhibit robustness,
despite regressions observed for this particular data point here.
% $\select = $ "k.keyword LIKE `\%sequel\%'" or "k.keyword = `marvel-cinematic-universe'". 

Increasing this sample size $S$ to 1,000 results in an average $\grave S$ increase to 34

PQO:
% This decision is informed by the understanding that \OurSys's analysis of the original query is applicable primarily to its neighboring queries. Given that only a small region of the query space benefits from robustness, storing a few plans is sufficient to maintain efficiency and effectiveness in handling similar queries.

At one extreme, \cite{purandaredimensionality, jayant2008identifying} diagram for the entire dimension space to identify robust plans, involving calls to the optimizer exponentially in the discretized resolution along each dimension.  Our method represents a middle ground and requires significantly fewer $\Opt$ calls. 




==> archive/conclude.tex <==
\section{Conclusion and Future Work}
Optimize a small faction of the query instances and store the plan and samples that works for the entire parameter space. Fully employ SRQO's pipeline in PostgreSQL to provide RQO at optimization time (online selection) even for a single query, e.g. the recost featuer in \cite{dutt2017leveraging}.


==> archive/error.tex <==
\section{error profile generation} \label{sec: err}
Most of the current selectivity estimators produce a single estimate without any indication of its uncertainty. The deep learning-based selectivity estimators have the ability to output the expected value as well as the variance. Although this straightforward normal distribution accounts for uncertainty, it may fail to accurately represent the true distribution of the potential selectivity errors. In practical scenarios involving query workloads, people tend to query popular values that are showing frequently in the query workload instead of a random value. In that case, a naive normal distribution may not work since it is constructed without any knowledge of the underlying workload. We argue that a high-quality error profile needs to be generated based on the specific workload.

Suppose we have a query workload, which involves numerous calls to execute query predicates. For each execution, we can observe both the actual selectivity and the virtual selectivity predicted by the selectivity estimator. In contrast to depending on a basic normal distribution, we construct a weighted distribution that takes the prevalence of the predicates into account. Specifically, we assign higher weights to those query predicates that occur frequently within the workload to emphasize their significance. While we monitor and track the errors that we have seen across the entire workload, we do not remember whether a particular error is associated with a specific predicate literal or not. Indeed, the potential selectivity of a query predicate is a function of both the estimated selectivity value and the potential error. An intuitive insight underscores that different estimated selectivity values should be applied with distinct error profiles; for instance, when the estimated selectivity is 0.1, it necessitates a different error profile compared to when the estimated selectivity is 0.001. We capture the relationship between the error profile and the estimated selectivity by tailoring error profiles to the specific estimated selectivity values. In essence, we bin the original error distribution into distinct error profiles. These partitions allow us to align the specific error profile with the selectivity estimation and improve the precision and granularity of our error modeling. Consequently, it equips us with a more accurate and refined understanding of uncertainty, paving the way for more insightful and adaptive decision-making in the realm of query optimization.

As showed in \ref{tab: q17-ori-dim}, the number of dimensions in a parameterized query could be exponential. Ideally, we should create error profile for each different dimension. However, this will not be realistic. This problem is similar to when the DBMS is maintaining high-dimensional statistics to estimate the selectivity of conjunctive predicates. These multivariate statistics, even it is a basic histogram structure, is too large to store. Therefore, in our context, we simplify the problem that we focus only on those dimensions related to single table relations and join relation between a pair of tables. For those complex join dimensions, we use the selectivity of the simplest join join relation's.

\textbf{Recentered Plan AND Use Error distribution to collect plan candidates}

==> archive/expr.tex <==
\section{Experiments}
\label{sec:expr}

All experiments were performed on a Linux server with 16 Intel(R) Core(TM) i9-11900 @ 2.50GHz processors. PostgreSQL V12.5 was used as the optimizer for end-to-end analyses. We use the Join Order Benchmark (JOB) \cite{job}, which contains 33 SQL queries with real-world data from Internet Movie Data Base (IMDB) . The dataset includes various join relationships that contain selectivity uncertainties. 
To obtain the actual execution time of each query, we executed each query 101 times and recorded the median result. We utilized the implementations from \cite{han2021cardinality} and \cite{pg_hint_plan} to inject the plan and selectivity errors as hints to PostgreSQL.

\subsection{Per Query Optimization}
\subsubsection{Build Error Profiles} 
To construct an error distribution for dimensions in a parameterized query, we narrow our focus to dimensions related solely to single table relations and join relations between pairs of tables as discussed in Section \ref{sec: err}. We simulate a query workload to obtain true error data, mirroring real-world conditions. 
We begin by gathering all potential predicate literals from the wrokload of JOB. Then, in the given query, for those single table relations with local selections conditions, we create a template that only involves that table and apply the possible predicate literals and then use a Gaussian kernel to estimate the PDF. 
Single-table relations lacking local selection conditions or containing only categorical tables with "=" predicates are disregarded since the optimizer will not make mistakes on these dimensions.
Moreover, for join selections, if a query involves a join between tables A and B, and either of these tables has local selection conditions, we should build the distribution learned from historical sub-queries that involving joining these tables with local selection conditions specified in the original query. In our experiments, we employ a template to join these tables and adjust the pre-collected local selection conditions accordingly. 
If neither table in a relation has local selections, we examine PostgreSQL's intermediate relations, particularly those involving 3-table joins. We determine whether the join relation will be utilized when another table with local selection conditions joins the original table first (e.g., (A join C) join B, where C has local selection conditions). Then we construct a 3-table join template to collect the data. Besides, if multiple 3-table joins meet these criteria, we build templates accordingly and collect all the error together to generate the PDF. If no 3-table joins meet the criteria, we simply join the two tables without any local selection conditions and collect the error. We show two examples in \ref{fig:err distribution} where \ref{fig: mc-cn} is a join relation between "mc" and "cn" with selection conditions on both tables and \ref{fig: mk-k} is table "mk" join "k" with selection condition only on table "k".


\begin{figure}
    \centering
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[scale=0.15]{figures/mc-cn-both-crop.pdf}
    \caption{mc-cn}
    \label{fig: mc-cn}
    \end{subfigure}
    \vspace{-3mm}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[scale=0.15]{figures/mk-k-r-crop.pdf}
        \caption{mk-k}
        \label{fig: mk-k}
    \end{subfigure}
    \caption{Simulated Error Distribution from JOB}
    \label{fig:err distribution}
    
\end{figure}

\subsubsection{Robust Plan Performance}
First, we compare the real execution latency to evaluate the performance of plan selected by SRQO for each single query. To analyze the sensitive dimensions, we choose Morris and Sobols method respectively, since the first is the extension of OAT method and the latter one is more capable to capture the interaction between different dimensions. We use $\mathcal{G}_1$ as our robustness metric and set the tolerance threshold $\sigma = 1.2$, which is a widely used and confirmed bound in several previous work \cite{harish2007production, 2018rqo, dutt2014plan, dey2008efficiently}, as we mentioned we do not wish to dictate a single notion of robustness measurement because it depends on the application scenario. 
We use the original optimal from PostgreSQL and the plan selected by WBM\cite{2018rqo} as our baselines. In the case of WBM, we incorporate the three proposed metrics by their work and highlight the best plan selection based on execution time. Instead of simplifying the problem by removing all local selection conditions on local tables in WBM, we opt to retain all of the original queries in the JOB dataset. Figure \ref{fig:exe-all}  displays the JOB queries along the x-axis, while the end-to-end query execution time for a plan $P$ is represented on the y-axis in milliseconds on a logarithmic scale. Additionally, the y-axis indicates the speedup or regression of each plan relative to the PostgreSQL plan. The speedup value is calculated by $(\textsf{latency of } P_{opt} / \textsf{latency of } P) - 1$, while, regression is defined as $1 - (\textsf{latency of } P / \textsf{latency of } P_{opt})$.
Across the entire set of 33 queries, SRQO outperforms PostgreSQL's plan in XX queries. For X queries, SRQO and PostgreSQL select the same plan, while neither SRQO nor WBM choose a better plan. In 5 queries, SRQO selects a plan that performs worse. As present in Figure \ref{fig:exe-good}, Sobol's method outperforms others in most cases. The most notable improvement in execution time is observed in Q17, where SRQO's plan takes 837 ms, while PostgreSQL's plan and the one selected by WBM take 5503 ms and 4030 ms, respectively.  In Q20, SRQO-Sobol achieves an execution time of 114 ms, a 8x speedup compared to PostgreSQL's plan with 1027 ms and WBM's plan with 955 ms. Morris' method, although not as effective as Sobol's, still surpasses WBM in most cases.



\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.57\linewidth}
    % \centering
    \includegraphics[scale=0.18]{figures/exe time/per-query-execution-time-all_with_speedup.pdf}
    \caption{Speedup}
    \label{fig:exe-good}
    \end{subfigure}
    \vspace{-3mm}
    \begin{subfigure}{0.37\linewidth}
        \centering
        \includegraphics[scale=0.18]{figures/exe time/per-query-execution-time-bad_with_speedup.pdf}
        \caption{Regression}
        \label{fig:exe-bad}
    \end{subfigure}
    \caption{\small{Actual execution time for different plans selected by various methods. Figure \ref{fig:exe-good} displays the queries for which SRQO selects a faster plan, while Figure \ref{fig:exe-bad} illustrates cases where SRQO's plan performs worse. The number in parentheses indicates the number of dimensions over the selectivity space. Other queries are omitted as SRQO selects a plan with nearly the same performance as PostgreSQL.}}
    \label{fig:exe-all}
    
\end{figure*}



\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[scale=0.23]{figures/injection.pdf}
    \caption{Optimization with exact selectivity}
    \label{fig:inject}
    \end{subfigure}
    \vspace{-3mm}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[scale=0.14]{figures/exe time/per-query-execution-time-quality.pdf}
        \caption{Quality of Err Distribution \haibo{Change Name?}}
        \label{fig:exact-and-quality}
    \end{subfigure}
    \caption{\small{Evaluate sensitive dimensions and the quality of error profile.}}
    \label{fig:ablation}

\end{figure*}

Among all queries, regardless of whether SRQO performs well or poorly, the robustness measurement used in WBM exhibits comparable performance to PostgreSQL. This is attributed to WBM's strategy of filtering out candidate plans with significantly higher estimated costs compared to the optimal plan at the given selectivity estimates, e.g., $\textsf{Cost}(P, \vec{S}) > \textsf{Cost}(P_{opt}, \vec{S}) * 1.2$. When the original plan is already optimal and robust at a particular selectivity point, WBM can easily select it by focusing solely on that local point without considering potential uncertainty, thus benefiting from this approach. 
However, SRQO constructs its candidate plan set by aggregating optimal plans across potential selectivity spaces, taking into account the uncertainties in selectivity estimation. And sometimes, a real promising plan may exhibit a much higher cost value than the original PostgreSQL plan. For instance, in the case of Q2, the default plan has a cost of 3,956, while SRQO's plan costs 40,325. Similarly, for Q17, the default plan costs 4,684, yet SRQO identifies the most robust plan using Sobols with a cost value of 124,610, nevertheless the cost is 27x higher, this plan performs exceptionally well. Our experiments highlight that even when a plan has a high estimated cost, we must consider it as a candidate because it may indeed be optimal, despite being overlooked by the cost model due to the unknown real selectivity at runtime.

\haibo{Discuss about recenter. Morris seems depend on recenter. Morris is OAT, it's better since we sample from error distribution.}

For queries where SRQO does not perform optimally, as presented in Figure \ref{fig:exe-bad}, we provide a breakdown of the reasons. For instance, in queries Q3 and Q4, both involve the condition \textit{k.keyword LIKE '\%sequel\%'}, the error distribution on the join relation of mk-k leads to an overestimation of the selectivity error. 

To further illustrate that the methods applied in SRQO can identify a more appropriate set of sensitive dimensions, we evaluate execution performance by sequentially incorporating actual selectivity values from the most to the least sensitive dimensions into the cost model. Subsequently, we instruct PostgreSQL to re-optimize the query, generating a new plan based on these precise selectivity inputs, a strategy also employed in \cite{chaudhuri2009exact}. Note that all subsequent experiments will utilize Q2, Q17, Q15, and Q26 as examples. These four queries are chosen to represent a spectrum of complexity, ranging from relatively simple with 5 tables joined to more complex queries involving up to 12 tables joined. Table \ref{tab:basic_info} and Figure \ref{fig:graph} provide basic information about these queries and illustrate the corresponding query graph and sensitive dimensions for each query. 
Figure \ref{fig:inject} showcases the outcomes of re-optimizing queries using exact selectivity values. For the dimensions identified by SQRO as sensitive, we progressively inject the exact selectivity of them in order of sensitivity, limiting our focus to the top three dimensions. Since WBM classifies non-foreign key joins as sensitive, we randomly choose three such dimensions and inject them sequentially. The final execution times of the plans by post-injection of all sensitive dimensions identified by WBM, are also presented. 
In Q2, Q17, and Q26, correcting the top three sensitive dimensions with both Sobol and Morris methods results in significant speed improvements, outperforming the results from WBM. WBM only matches these improvements in Q26 after all its identified sensitive dimensions have been corrected. In Q15, none of the methods, including Sobol, Morris, or WBM, improve upon the original PostgreSQL plan, indicating that the initial plan was already robust. 
We further explore the impact of error profile quality on SRQO's performance , examining five distinct scenarios in the "error-aware" setting. Initially, in the absence of any assumption about potential selectivity errors, we default to relying on PostgreSQL's planning, which serves as our baseline. Subsequently, we consider the naive assumption, as suggested in \cite{abhirama2010stability, chaudhuri2010variance}, that errors could span the entire parameter space, resulting in the selectivity distribution randomly scattered across a broad range for each dimension; this scenario is denoted as "LEC" (Least Expected Cost). In our approach, we compile historical error data to construct error profiles. The "Simplest" profile employs the entire error dataset but simplifies its representation to a Gaussian distribution using just the mean and standard deviation. The final two are constructed using 1\% and 100\% of the error data, respectively, to develop the error model. 
The results depicted in Figure \ref{fig:exact-and-quality} indicate that "LEC" only yields small improvements for Q17, failing to perform well on the other queries. This underscores the importance of focusing on sensitive dimensions and quantifying the error. "Simplest" and "1\% data" demonstrate better performance than "LEC" but are not as effective as "100\% data" for Q2, Q17, and Q26. The reason is both "Simplest" and "1\% data" lack comprehensive information compared to "100\% data." However, in the case of Q15, "1\% data" outperforms "100\% data" because the synthetic error distribution is still differing from exact real-world scenarios. Using a smaller dataset to construct the distribution helps mitigate this discrepancy.



\haibo{Add: Overhead and Samples required to converge!!!}

\begin{table*}[]
    \centering
    \begin{tabular}{cccc}
        \hline
        \textbf{Q id (\# of Dimensions)} & \textbf{Sobols input sample (from distribution)} & \textbf{Sobols samples (simulated)} & \textbf{Top 3 Sensitive Dims} \\
        \hline
        2 (5) & 16 & 192 & (mc cn), (mk k), (mk mc) \\
        17 (12) & 64 & 1664 & (mk k), (mk ci), (n ci) \\
        26 (21) & 256 & 11264 & (mi\_idx, it), (t cc), (mi\_idx, cc) \\
        15 (18) & 64 & 2432 & (mc cn), (t aka\_t), (mc aka\_t) \\
        \hline
    \end{tabular}
    \caption{Samles required to Converge sobols}
    \label{tab:converge}
\end{table*}
In the following sections, we will demonstrate the robustness of the plans selected by SRQO and also illustrate that even when a plan does not perform as well as the optimizer's plan in the per query settings, it can still function effectively when the query's predicates vary in the Parametric Query Optimization setting.



\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{figures/query-graph/Q2-graph-cropped.pdf}
    \ \ 
    \includegraphics[scale=0.3]{figures/query-graph/Q17-graph-cropped.pdf}
    \ \
    \includegraphics[scale=0.3]{figures/query-graph/Q26-graph-cropped.pdf}
    \ \
    \includegraphics[scale=0.3]{figures/query-graph/Q15-graph-cropped.pdf}

    \caption{Query Graphs of Q2, Q17, Q26 and Q15 \haibo{maybe highlight sensitive dims?}}
    \label{fig:graph}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.14]{figures/cdf/2apenalty_cdf_sen_dim_all_plan.pdf}
    \ \ 
    \includegraphics[scale=0.14]{figures/cdf/17apenalty_cdf_sen_dim_all_plan.pdf}
    \ \
    \includegraphics[scale=0.14]{figures/cdf/26apenalty_cdf_sen_dim_all_plan.pdf}
    \ \
    \includegraphics[scale=0.14]{figures/cdf/15apenalty_cdf_sen_dim_all_plan.pdf}

    \caption{Cumulative Density Function of Cost Penalty for Q2, Q17, Q26 and Q15}
    \label{fig:cdf}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.105]{figures/verify/verify-2-sample-4.pdf}
    \ \ 
    \includegraphics[scale=0.105]{figures/verify/verify-17-sample-4.pdf}
    \ \
    \includegraphics[scale=0.105]{figures/verify/verify-26-sample-4.pdf}
    \ \
    \includegraphics[scale=0.105]{figures/verify/verify-15-sample-4.pdf}

    \caption{Robustness Verification on Multiple DB Instances by Sliding Window on Time Series Data. The instances are created from the original IMDB database by a sliding window on  \textit{production\_year}. 
    We use SRQO to select the most robust plan only on DB5 and evaluate the performance of this plan on the other DB instances. }
    \label{fig:verify-slide}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[scale=0.105]{figures/verify/verify-2-cat-1.pdf}
    \ \ 
    \includegraphics[scale=0.105]{figures/verify/verify-17-cat-1.pdf}
    \ \
    \includegraphics[scale=0.105]{figures/verify/verify-26-cat-1.pdf}
    \ \
    \includegraphics[scale=0.105]{figures/verify/verify-15-cat-1.pdf}
    \\
    \includegraphics[scale=0.105]{figures/verify/verify-2-cat-5.pdf}
    \ \ 
    \includegraphics[scale=0.105]{figures/verify/verify-17-cat-5.pdf}
    \ \
    \includegraphics[scale=0.105]{figures/verify/verify-26-cat-5.pdf}
    \ \
    \includegraphics[scale=0.105]{figures/verify/verify-15-cat-5.pdf}
    \caption{Robustness Verification on Multiple DB Instances by Categorical Partitioning. The instances are partitioned from the original IMDB database by \textit{kind\_type.kind}. 
    We choose "Movie" and "Video Game" as the base instance respectively.}
    \label{fig:verify-category}
\end{figure*}

\subsubsection{Verify Robustness} 
\paragraph{\textbf{Cost Penalty Distribution}}
First, we aim to understand why certain plans are elected as the most robust and explore the distribution of cost penalties associated with their selection. For each query, we utilize the samples from SRQO's robustness metrics calculation to generate Cumulative Density Function (CDF) for plans selected by different methods, as present in Figure \ref{fig:cdf}. 
One primary criterion for selecting robust plans is minimizing significant cost penalties. Across all queries, plans chosen by SRQO exhibit substantially lower occurrences of large cost penalties compared to those selected by alternative methods. 
Although it's worth noting that these robust plans may sometimes incur smaller penalties, such as in the case of Q26 where WBM and Recenter have approximately 60\% of samples with penalties less than $10^3$, while SRQO only has around 30\% of them. Similarly, for Q15, unlike all the others which have nearly 50\% of samples with penalties less than $10^4$, SRQO barely has any. However, SRQO's plan excels precisely at those points in the selectivity space when the other plans perform extremely poorly with notably high cost penalties.
\paragraph{\textbf{Verify Robustness on Multiple DB Instances}}
The results presented in Figures \ref{fig:exe-all} are obtained using the entire IMDB dataset. However, since a DB instance has a fixed selectivity error for each predicate, relying solely on the performance of a single instance cannot sufficiently demonstrate robustness. We aim for the robust plan to demonstrate resilience against unpredictable selectivity uncertainties. Therefore, to simulate the unforeseen selectivity errors encountered in real-world scenarios, we generate multiple DB instances. We apply SRQO to identify the most robust plan on one instance and evaluate this plan on other instances without prior knowledge of their selectivity errors. Additionally, we execute two comparison plans: one selected by PostgreSQL on the base instance and another selected by calling PostgreSQL on the specific instance. These comparison plans serve as benchmarks for evaluating the effectiveness of the SRQO-selected plan with different selectivity errors.
\begin{itemize}
    \item Sliding Window on Time Series Data: We sort the \textit{title} table based on the \textit{production\_year} attribute and construct a new database instance by sampling 20\% of the data from \textit{title} along with corresponding data from other tables. Starting with the initial 20\% of data from the sorted table, we create 9 instances by sliding this window by 10\% at each step, labeled as DB1 to DB9. We regard DB5 as our base instance and evaluate the plan selected by SRQO on other instances.
    
    \item Categorical Partitioning: We partition the original database by item’s \textit{kind\_type.kind} into 6 new instances, representing different categories such as "Movie", "TV Series", "TV Movie", "Video Movie", "Video Game", and "Episode", (we excluded the "TV Mini Series", since it has no rows) resulting in a total of 6 instances, represented by the corresponding category name. In this method, we choose the largest instance "Movie" and the smallest "Video Game" as the base instance, while the remaining instances are treated as testing instances. Details of the created DB instances are present in Table \ref{tab:cat}.
\end{itemize}
We first present the performance results on DB instances created by sliding window, in Figure \ref{fig:verify-slide}. Despite already achieving better performance on the base instance DB5 for queries Q2, Q17, and Q26, our plan consistently outperforms both the new plan selected by PostgreSQL and its original plan from DB5, across all other DB instances. 
For Q15, although SRQO's selected plan is not the optimal one for DB5, it demonstrates robust performance on other instances, even outperforming the optimizer's new plan in 4 cases (DB3, DB4, DB8, and DB9). On DB6 and DB7, where the selectivity error distributions of these neighbor instances are probably similar to the base instance, our plan is slightly slower compared to the optimizer's plan.
Besides, on DB1 and DB2, our plan avoids significant performance degradation, unlike the original PostgreSQL plan.

To create more challenging variations in selectivity uncertainty, we employ our second partitioning method, which divides the original databases into six new segments by "kt.kind". Based on the average row size in these instances, we selected "Movie" and "Episode" as the base instance, representing the largest and smallest instances, respectively, while the others served as testing instances. The originally Q26 includes a predicate on the kind\_type table as "kt.kind = `moive' ". We modify this condition to "kt.kind IS NOT NULL" to avoid selecting 0 rows, which would be meaningless. 
When examining Q2 and Q17, we observe similar performance trends as with the previous partition method, as illustrated in Figure \ref{fig:verify-slide}. The plans selected by SRQO on the base instance effectively mitigate selectivity errors and perform well on all of the testing instances, outperforming the new plans generated by PostgreSQL. We find that the overall execution time when using the plan based on "Video Game" is worse than when using "Movie," it is because "Movie" is larger and the statistical information in that database instance is more reliable.
When "Movie" is regarded as the base instance, for Q26, SRQO's plan still leads to speedup on the base instance but results in regression on the testing instances. The reason is that the selectivity error on these testing instances might be too different from the error profile built from "Movie". However, our robust plan avoids the dramatic sub-optimality made by the original PostgreSQL plan on "TV Series" and "Episode."
For Q15, SRQO selects a plan which is slightly worse on the base instance but avoids unacceptable behavior on "Video Movie," demonstrating that our plan is more error-resistant. When we use SRQO to select the plan for Q26 on "Video Game," our plan shows similar performance compared with the original PostgreSQL's plan on most instances, while our plan performs better on "Episode" where the regression is significant for both testing plans. For Q15, we select the same plan as PostgreSQL, and the largest regression is 1.3 among testing instances, indicating that the original plan by PostgreSQL is already robust.


\begin{table}[]
\begin{small}
\centering
\begin{tabular}{p{0.7cm}p{0.8cm}p{1.0cm}p{0.9cm}p{0.9cm}p{0.9cm}p{0.8cm}}
\hline
& Movie & TV \hspace{0.3cm} Series & TV Movie & Video Movie & Video Game & Episode \\
\hline
 t & 663k & 91k & 101k & 118k & 13k & 1543k \\
 mc & 1308k & 194k & 200k & 160k & 30k & 717k \\
 mk & 2887k & 183k & 251k & 473k & 85k & 645k \\
 ci & 10397k & 889k & 1950k & 1378k & 211k & 21420k \\
 % ml & 0 & 12k & 0 & 0 & 0 & 18k \\
 mi & 8301k & 770k & 804k & 883k & 115k & 3963k \\
 cc & 60k & 3k & 8k & 3k & 65 & 62k \\
 at & 293k & 20k & 27k & 13k & 5k & 3k \\
 miidx & 630k & 113k & 111k & 84k & 17k & 426k \\
 k & 111k & 25k & 34k & 27k & 12k & 65k \\
 cn & 188k & 31k & 28k & 27k & 5k & 12k \\
 % an & 637k & 87k & 150k & 106k & 12k & 290k \\
 n & 637k & 87k & 150k & 106k & 12k & 290k \\
 % pi & 748k & 363k & 526k & 338k & 78k & 644k \\
 % lt & 0 & 16 & 0 & 0 & 0 & 15 \\
 it & 95 & 92 & 92 & 93 & 53 & 57 \\
 ct & 2 & 2 & 2 & 2 & 2 & 2 \\
 kt & 1 & 1 & 1 & 1 & 1 & 1 \\
 chn & 1699k & 164k & 370k & 132k & 41k & 1185k \\
 % rt & 11 & 11 & 11 & 11 & 11 & 11 \\
 cct & 4 & 4 & 4 & 4 & 3 & 4 \\
\hline
\end{tabular}

\caption{Information of Created DB Instances. New instances from DB1 to DB6 are partitioned by \textit{kind\_type.kind} to imitate the unknown selectivity errors in the practical situation. Only tables involved in representative queries Q2, Q17, Q26, and Q15 are listed, while others are omitted.}
\label{tab:cat}
\end{small}

\end{table}

\subsubsection{Ablation Study}
\subsection{Parametric Query Optimization}
\textbf{Build Query Template} First we construct a template SQL query using the overall structure of the target query. Then we make this template flexible to accommodate parameter bindings, to be specific, varying conditions on individual tables. In our experimental setup, again we use the collected possible literals from JOB. These literals are then applied to their corresponding tables, following their respective distributions, to generate a comprehensive array of query instances. 
Furthermore, we eliminate corner cases where certain combinations of predicate literals yield nonsensical results, such as instances where the output of a combination produces zero rows. In practice, when the optimizer detects a table producing zero rows, it typically avoids executing subsequent join relations, thus saving execution time. Consequently, the execution time becomes uncorrelated from the estimated cost. Additionally, when a query plan is hinted, the optimizer is compelled to follow the hinting, thus, we are unable to monitor the end-to-end behaviors of plan candidates in a fair manner.\\
\textbf{Settings}: 
For the experiment setup in the PQO settings, we adopt the following parameters:
\begin{itemize}
    \item Robust Plan Caching: We cache a limited set of robust plans, typically up to three, derived from the analysis of the preceding single query. This decision is informed by the understanding that SRQO's analysis of the original query is applicable primarily to its neighboring queries. Given that only a small region of the query space benefits from robustness, storing a few plans is sufficient to maintain efficiency and effectiveness in handling similar queries.
    \item Samples Caching: Our experiments indicate that caching 100 samples is sufficient to achieve satisfactory performance.
    \item Number of Generated Queries: We generate 100 queries from our query template. These queries represent a diverse set of database operations and scenarios, providing a comprehensive evaluation of the PQO approach.
    \item Dimension Consideration: All dimensions are considered when calculating the Kullback-Leibler (KL) divergence and the probability of being sampled. This ensures that the analysis accounts for the variability across all dimensions, capturing the overall distribution of the error samples and their impact on query optimization.
\end{itemize}

Results are showed in Table \ref{pqo}. \haibo{Add analysis of Figure \ref{fig:latency-cdf} and Table \ref{pqo}} 

Latency distribution of 4 selected queries are displayed in Figure \ref{fig:latency-cdf}. For the low hit rate, the reason lies in the significant discrepancy between the estimated selectivity of predicates used in the original query and the majority in the collected predicates. It will be our future work to extend SRQO's application to multiple query instances, thereby covering the entire relational selectivity space of the parameterized query.

\begin{figure}
    \centering
    \includegraphics[scale=0.22]{figures/cdf/latency cdf/q7-latency-cdf.pdf}
    \ \ 
    \includegraphics[scale=0.22]{figures/cdf/latency cdf/q17-latency-cdf.pdf}
    \\
    \includegraphics[scale=0.22]{figures/cdf/latency cdf/q26-latency-cdf.pdf}
    \ \
    \includegraphics[scale=0.22]{figures/cdf/latency cdf/q18-latency-cdf.pdf}

    \caption{Cumulative Density Function of Execution Time in PQO for Q7, Q17, Q26 and Q18}
    \label{fig:latency-cdf}
\end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.18]{figures/exe time/pqo-execution-time-all_with_speedup.pdf}
    \caption{Summary of PQO Results}
    \label{fig:pqo}
\end{figure*}


==> archive/framework.tex <==
\section{Overview}
\subsection{Problem Overview}
In parametric query optimization, the estimated cost of a query plan is calculated as a function of various selectivity estimations. Given a set of selectivity parameters, the traditional query optimizer aims to search for an execution plan with the lowest estimated cost from the candidate plan set. However, such a choice might be highly sensitive to errors in selectivity estimation, because the estimated cost is calculated only based on point selectivity estimates. In this paper, we argue that this problem can be addressed by finding a robust plan that takes the uncertainty of selectivity estimation into account. As shown in Figure \ref{fig:q17}, we use Q17 from Join Order Benchmark\cite{job} (JOB) as examples to explain the need for a robust plan. Q17 joins 7 tables as showed in Figure \ref{fig: q17-graph},  where each node corresponds to an individual table and each edge represents the join key linking two tables. To show the necessary of choosing a more robust plan, we build 9 database instances from DB1 to DB9 (details for instances construction are present in section \ref{sec: exp}) and consider the middle instance DB5 as the base instance, analyze the most robust plan choice only on DB5, but test it on the other instances from DB1 to DB9, except DB5, to mimic the unknown selectivity estimation errors. Then we compare the performance of the most robust plan from DB5 with the optimizer's solution given by the call on each specific instance. Figure \ref{fig: q17-robust-behavior} shows that if we simply rely on the plan selected by the optimizer, the performances are really poor on all DB instances. To avoid picking a sub-optimal plan as the final decision, it is necessary to pay efforts to find a robust plan that can resist uncertainties. 


\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[scale=0.3]{figures/q17-graph.pdf}
    \caption{Query Graph}
    \label{fig: q17-graph}
    \end{subfigure}
    \vspace{-3mm}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[scale=0.25]{figures/verify-q17-0.2-intro.pdf}
        \caption{Robust Plan's Behavior}
        \label{fig: q17-robust-behavior}
    \end{subfigure}
    \caption{Example on q17. (a) The visualized join graph. (b) Why do we need a robust plan instead of using the optimizer's default plan? The real performance of the optimizer's plan on each DB instance VS the most robust plan found on DB5.}
    \label{fig:q17}
    
\end{figure}

\subsection{Problem Defnination}
To formally define the problem, let's consider a query $Q$ with a set of $d$ parameterized selectivity values. These selectivity values can be represented as a point in a $d$-dimensional space, denoted by $\vec{S} = \{ s_1, s_2, ..., s_d\}$. Each value $s_i$ indicates the proportion of rows in a table or join that satisfy the corresponding predicate. For each possible execution plan $P$ of $Q$, the optimizer uses a parameterized cost function to evaluate its efficiency. The cost function takes the potential plan $P$ and the selectivity combination $\vec{S}$ as the input parameters and returns the estimated cost (without execution) of $P$, notated as  $\textsf{Cost}(P, \vec{S})$. The cost function has the same dimension as the number of selectivity parameters. The physical plans we are considering are with different join orders, join methods and scan methods. We leverage the existing cost-based query optimizer to calculate the value and regard the cost model as a black box since the function is complex and opaque to the parameters. Following the assumption in several previous works (plan bouquets serious), we also assume this cost value can be precisely calculated by the cost model. Our experiment also demonstrated that there is a strong correlation between the cost model and the running time, which is consistent with \cite{job}.


\begin{definition} Given a query $Q$, let $\mathbb{P}(Q)$ be the set of all possible execution plans. Then, the optimizer will search for the one in $\mathbb{P}(Q)$ with the minimum cost, 
\begin{equation}
     \arg \min_{P \in \mathbb{P}(Q)} \textsf{Cost}(P, \vec{S})
\end{equation}
and return it for the user to execute. 

However, due to the limited learnability of current selectivity estimation models, it is hard to accurately estimate the selectivity value. The errors contained in cardinalities might result in the plan chosen by the optimizer being sub-optimal or even poor. Given the truth that the error of estimations is unavoidable, we claim to make the optimizer aware of the selectivity uncertainties and then select the most robust plan based on the potential errors instead of the point estimates only.
\end{definition}
\begin{definition}
Suppose $\vec{E} = \{ e_1, e_2, ..., e_d\}$ is the potential selectivity errors on each dimension in $\vec{S}$. To capture the error distribution of each dimension, we define $F(\vec{E})$ as the joint probability density function (PDF) of potential errors $\vec{E}$. $F(\vec{E}) = \prod_{i=1}^{d} f_{i}(e_{i})$, where $f_{i}(e_{i})$ is the PDF of selectivity error on dimension $i$. $F(\vec{E})$ can describe the joint distribution of the selectivity error on $d$ predicates, and the boundary of this error distribution is a hyper-rectangle with $d$ dimensions, notated as $\mathbf{Z}$, i.e, $\vec{E} \in \mathbf{Z}$. The following conditions must be satisfied:

\begin{equation}
    \forall i \in [0, d], f_{i}(e_i) > 0 \text{, and} \int_{\mathbf{Z}_{i}} f_{i}(e_{i}) \ de_{i} = 1\\
\end{equation}
\begin{equation}
    \forall \vec{E} \in \mathbf{Z}, F(\vec{E}) > 0 \text{, and} \int_{\mathbf{Z}} F(\vec{E}) \ d\vec{E} = 1\\
\end{equation}
The distribution of selectivity errors allows us to quantify uncertainties, and our ultimate goal is to make the optimizer aware of these uncertainties and select a plan that is resilient to such errors. Section \ref{sec: err} will introduce how we collect the real error data from the historical executions and how to build the error distribution. In this paper, we are particularly interested in understanding and identifying those critical components where uncertainties can significantly impact the final performance and plan choice. We refer to these critical components of the query as "sensitive dimensions" that require extra attention and effort to ensure a robust outcome.


\end{definition}
\subsection{Framework of SRQO}
Again we use Q17 to illustrate the framework of SRQO. For this target query, we can extract a total of 56 sub-queries. These sub-queries comprise individual tables and their associated join relations. During the query optimization procedure, the cost function requires the selectivity estimation of each sub-query to measure the cost of plans, which results in a high dimensional space. Based on the propagation relations, we simplify the problem to only consider the local selection conditions and the conditions related to pairs of join relations as our dimensions. Because the selectivity of more complex join relations can be computed using the simpler selectivities. In this case, we denote the dimension of the parameterized cost function as $dim(\textsf{Cost}) = 16$. 

The initial step in our framework involves building an error distribution for each relation. These error distributions are crucial for subsequent analysis. Section \ref{sec: err} provides a detailed outline of the error profile construction procedure. Following this, the next step of SRQO is to identify the sensitive dimensions. In other words, our objective is to filter out dimensions that do not affect the final plan decision, even in the presence of estimation errors on those dimensions. For instance, when applied to Q17, SRQO identifies 4 dimensions from the original set of 16 dimensions, including \haibo{[updated from new converged experiments]: (mk k), (mk ci), (ci n)}. We discussed our proposed method to analyze the sensitive dimensions in Section \ref{sec: sen-dim}. Next, SRQO builds a candidate plan pool, and ensure each plan in this pool is either near-optimal or optimal in some selectivity estimation values with regard to the uncertainty distribution. Then we propose three alternative robustness metrics based on the application scenario to evaluate the robustness of each plan with the awareness of potential selectivity uncertainties and finally select the plan with the lowest robustness value as the our solution. Details are present in Section \ref{sec:metrics}. After the responsive optimization for a single query, in a parametric query settings, SRQO can also reuse the cached information for other queries with same structure but different parameter instantiations.


\begin{table*}[t]
% \setlength{\tabcolsep}{8.9pt}
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Base Tables} & \textbf{2-tables Join} & \textbf{3-tables Join} & \textbf{4-tables Join} & \textbf{5 to 7 tables Join} \\
    ci & (mc ci) & (cn ci mc) & (mk ci cn mc) & (k ci cn mc mk)\\
    cn & (mk ci) & (mk ci mc) & (n ci cn mc) & (n ci cn mc mk) \\
    k & (n ci) & (n ci mc) & (k ci mc mk) & (t ci cn mc mk) \\
    mc & (t ci) & (t ci mc) & (n ci mc mk) & (t ci cn mc n) \\
    mk & (mc cn) & (k ci mk) & (t ci mc mk) & (n ci k mc mk) \\
    n & (mk k) & (n ci mk) & (n ci k mk) & (t ci k mc mk) \\
    t & (mk mc) & (t ci mk) & ... & ... \\
     & (t mc) & (t ci n) & ... & ... \\
     &  & (mk cn mc) & ... & ... \\
  &  & (t cn mc) & ... & ... \\
   &  & (mc k mk) & ... & ... \\
    &  & (t k mk) & ... & ... \\
  &  & (t mc mk) & ... & ... \\
    7 dims & 9 dims & 13 dims & 13 dims & 14 dims \\
\hline
\end{tabular}

\caption{Dimension Categories in Q17. In total, we have 56 dims. Each is a dimension in the cost function.}
\label{tab: q17-ori-dim}
\end{table*}


==> archive/intro.tex <==
\section{Introduction}

Traditional query optimizers use estimated costs from a cost model to guide their decision-making. Given a query, the cost model can be regarded as a parameterized function that takes the selectivity values of each sub-query as input, including the predicates on individual tables and intermediate join results. Research has shown that current cost models are generally effective at measuring the execution cost of a given query plan, and even simple cost models can provide accurate measurements \cite{scheufele1997complexity, job, yang2022balsa}. Instead, the quality of solutions from these cost modles is heavily dependent on the accuracy of the input selectivity parameters. Even a small error in the basic information can lead to significant propagated errors, particularly as the number of joins increases \cite{ioannidis1991propagation}. Such uncertainties may result in sub-optimal decisions when selecting a plan, and it remains unclear which errors are more likely to lead to these sub-optimal decisions.

Recent research has concentrated on improving the accuracy for a long period, such as developing learning-based methods to predict selectivities \cite{} avoiding the limitations of traditional statistics moethods, e.g. histogram \cite{} and sample from data \cite{}. However, precise estimation of selectivity remains an unsolved problem. Given the inherent unreliability of selectivity estimates, the compromise solution is to develop a responsive optimization process that is flexible to input parameter uncertainties while mitigating sub-optimality. \haibo{** Revise below}

Although some other studies have introduced different metrics to evaluate the robustness of query plans, e.g. calculate the slope of the cost function or the integral within defined upper and lower bound of selectivity values, none of these approaches provide a comprehensive quantification of the potential errors and their consequential impacts.

In this project, we proposed SRQO which tries to capture the potential selectivity errors and optimizes the plan selection under the selectivity-error-aware settings. SRQO regards the cost model as a black box and defines Responsive Query Optimization as a workload-sensitive notion. For a given query workload, SRQO tracks the real selectivity errors from the historical query executions and leverages these data to construct a weighted probability density function (pdf) that characterizes the distribution of these errors on different selectivity of parameters. These error profiles grant us the ability to factor in the uncertainty associated with selectivity parameters during the query optimization process, despite the inherent challenge of capturing actual errors at run-time. 
Then we define the \textit{penalty} of choosing a sub-optimal plan as the difference between the cost of the real optimal plan and the cost of the plan that was chosen. This formulation allows us to quantify the repercussions of any decision-making punishment by the difference between the cost of the selected and the optimal plans. Based on the cost penalty and the error profiles, SRQO considers the interaction between all of the parameters and identifies a set of sensitive ones from the given query. We claim that these sensitive parameters necessitate more attention from the DBMS users to understand their potential error and ensure the accuracy in their estimations. To determine the most robust and efficient query plan, we proposed three alternative metrics that go beyond the traditional estimated costs only. Our metrics are effective for assessing plan robustness by not only taking into account the expected cost penalty value but also factoring in the variability of this penalty, which stems from the uncertainty associated with selectivity errors. We show that the plan selected by us exhibits better performance in terms of latency, as well as displaying remarkable resilience w.r.t unforeseen selectivity errors. Furthermore, our experiments demonstrate that our selected robust plan based on the original query also perform well in a parametric query optimization setting by caching the what we learned from the robustness analysis. 


==> archive/related.tex <==
\section{Related Work}
\label{sec:related}


\textit{Robst Query Optimization} 
The problem of query optimization has a long history, given that the sensitivity of decision models to uncertainties, finding an optimal plan remains a challenge even for those mature commercial DBMS. Therefore, how to improve the ability of error resistant and avoid sub-optimal risks for current optimizer has been widely discussed \cite{borovica2017robust, graefe2012robust, haritsa2019robust}. Robust query optimization can be regarded as part of robust query processing and is classified by the number of plan provided by a recent survey \cite{yin2015robust}. 
For single-plan based approach, many different methods to select the most robust plan has been proposed. The Least Expected Cost (LEC) \cite{chu1999least} was among the first to utilize probability density for estimating selectivity, aiming to identify plans with the lowest expected cost. However, LEC restricts the search space of plans and lacks a clear methodology for constructing probability measures, and its focus is primarily on identifying plans robustly executable in uncertain runtime environments. 
Similarly, \cite{abhirama2010stability, chaudhuri2010variance} pick a plan that has low variance and minimum average cost over extremes for the entire parameter space. However, the performance of these methods is limited since the error can not be captured in an arbitrary large selectivity space. In this paper, we present a concrete way to quantify the uncertainty and focus our attention on sensitive parameters only.
In contrast, the Robust Cardinality Estimation (RCE) method \cite{babcock2005towards} employs a set of samples from real underlying data to infer actual selectivity, using a user-defined confidence threshold. Unlike SRQO, which accounts for all possible uncertainties, RCE aims to leverage underline data and user knowledge to enhance selectivity estimation and avoid errors.
Rio \cite{babu2005proactive} and its extension \cite{ergenc2007robust, alyoubi2016database} leverage bounding boxes (intervals) to quantity the uncertainty of selectivity, and collect the plan as candidate if the cost is close to optimal over the bounding box. When executing the query, these candidate plans can be utilized as alternatives if re-optimization is necessary, rather than generating a new plan for the remainder of the query. The idea of adaptive processing query, e.g. collect running time observations and then switch the execution plan to another is also leveraged in \cite{dutt2014plan, dutt2014quest, trummer2021skinnerdb}. These interval-based approaches need to assume that predicate selectivity is known with in a narrow intervals, which is often violated in practical situation \cite{job}.
Besides, research on plan diagrams \cite{harish2007production, jayant2008identifying} aims to identify a fine-grained set of plan candidates for a query template across the relational selectivity space, each candidate can be regarded as a robust plan for certain area. Subsequent works \cite{purandaredimensionality, dey2008efficiently} present methods to reduce the complexity of the diagram, but they still necessitate time-consuming offline training through repeated invocations of the query optimizer. Additionally, the final plan selection is still reliant on point estimation of selectivity, which may lead to sub-optimal outcomes. 

Risk Score \cite{phdthesis2016} employs the coefficient of variation to measure the robustness of execution plans. However, this metric requires real execution times under various actual selectivity values. Furthermore, their model confines the variability in execution conditions to a single parameterized predicate, limiting its generality. 
Maximum Sub-Optimality (MSO)\cite{dutt2014plan, purandaredimensionality, jayant2008identifying, karthik2018concave} is widely used in robust query processing that quantifies the worst-case sub-optimality ratio across the entire predicate selectivity space. It relies on the availability of the real optimal plan, which is typically only known to the optimizer after the query execution has begun. 
WBM \cite{2018rqo} defines sensitive dimensions as non foreign key joins and presents three alternative metrics that only based on estimation to explicitly measure the robustness. The first two calculate the sum of slopes for all sensitive dimensions, while the last one is defined as the sum of the integral of cost for each sensitive dimension. The robustness metrics used in SRQO follow this direction that only based on estimation without running the query and evaluate each plan independently.

\textit{Parametric Query Optimization}
PQO has been a subject of study for three decades \cite{hulgeri2002parametric, ioannidis1997parametric}. The primary focus of PQO is to minimize the need for the optimizer's invocation by utilizing cached plans while ensuring that the resulting plan's cost remains acceptable. According to \cite{dutt2017leveraging}, current PQO methods can be classified based on the plan identification phase, which includes online-based and offline-based methods. 
For online-based methods, \cite{alucc2012parametric} builds a density map by clustering executed queries and plans, enabling the selection of a cached plan for any new query. The concept of clustering queries is also utilized in \cite{ghosh2002plan}. A recent study \cite{dutt2017leveraging} introduces "re-cost" to efficiently calculate any $\textsf{Cost}(P, \vec{S})$, thereby reducing overhead. The effectiveness of "re-cost" is demonstrated in \cite{dey2008efficiently}, where the ratio between plan-costing and plan-optimization is approximately 1:100. "re-cost" is also employed in SRQO for evaluating plan robustness.
For offline-based methods, the objective is to identify a set of plans that can ensure optimal execution performance for any instance across the selectivity space \cite{hulgeri2002parametric, ioannidis1997parametric}. The plan diagram introduced in \cite{harish2007production, picaso} is applicable in this setting.
A novel framework for PQO, decoupling candidate plan generation and learning-based plan selection, has been recently proposed \cite{vaidya2021leveraging, doshi2023kepler}. Typically, these approaches require collecting actual execution times for all candidate plans, then train a learning model to predict the best plan for any new query instance. Candidate plans in \cite{vaidya2021leveraging} are searched from executed queries, while in \cite{doshi2023kepler}, they are generated by randomly perturbing the cardinality of different dimensions, which is similar to our method of building the candidate plan set during robustness evaluation. However, SRQO focuses on sensitive dimensions and samples from the error distribution directly. \cite{doshi2023kepler} demonstrates that learning from real execution costs can accelerate PQO, offering a promising avenue for future research.
Currently, SRQO can serve as an offline plan caching and online plan selection method, and it can readily be extended to cover the entire selectivity space using techniques such as clustering \cite{alucc2012parametric, ghosh2002plan} or plan diagrams \cite{picaso}. However, the primary goal of this paper is not to outperform existing PQO methods; our focus is on leveraging robust plans from a base query instance for neighboring queries from the same query workload. Even without necessitating real execution times of query instances, SRQO can still enhance the overall performance by considering selectivity uncertainties and avoid optimizer calls.


\paragraph{1. Selectivity Estimation} Short: \\
1.1 Methods to improve the accuracy, query driven, data driven, learning\\
1.2 Uncertainty of Cardinality Estimation\\



==> archive/robust.tex <==
\section{Robustness Metrics} \label{sec:metrics}
In this section, we propose a new approach to improve the robustness of traditional query optimization by utilizing the selectivity error distribution. The traditional optimizer's decision for a query plan is typically based only on point estimates, which can contain many uncertainties. It is necessary to design some metrics that can guide us in choosing a robust plan that is resistant to selectivity uncertainties since these potential errors are often unavoidable and can have a significant impact on the actual performance of the chosen plan. Again, due to the fact that it is impossible to know the exact selectivity value at run time, we want the optimizer to make the decision based on estimated selectivities and the distribution of potential errors. 
Unlike previous works such as \cite{2018rqo, abhirama2010stability, chaudhuri2010variance}, we do not solely rely on point estimates or spread our focus across the entire selectivity space. Instead, we adopt a similar approach that calculates the expected value using the probability density function, enabling us to quantify the potential distribution of selectivity errors.
We introduce three alternative metrics to measure the robustness of query plans, each of which aims to find the most robust plan based on a different definition of robustness based on the application scenario. \haibo{\textbf{Change the space we used here to sensitive dim, instead of all dims.}}

\subsection{Robustness Based On Expected \textsf{Cost} Penalty}
A recently proposed robustness metrics \cite{2018rqo} typically evaluate the behavior of a plan by only analyzing the slope and integral of the cost function. However, these approaches may not always provide sufficient information to accurately assess the robustness of a plan. \haibo{Do we need a x-y 2-d plot here?} shows that the slope or integral of the cost function as the robustness value can not reflect if the plan is more robust than the other. Instead, we believe that robustness evaluation should focus on how \textit{poorly} a plan could perform. Likewise, even if the selected plan is not optimal, we may still consider it if its performance is not significantly worse. Therefore, to better understand plan robustness, it is more effective to identify the region where a wrong plan decision, as determined by the selectivity error, results in a penalty. Using a similar idea when we analyze the sensitive predicates, our first robustness metric is defined as the expected cost penalty using the selectivity error distribution.
\begin{definition} \textbf{Expected \textsf{Cost} Penalty} The expected cost penalty over the joint selectivity error distribution w.r.t the tolerance threshold is
    \begin{equation}
        \begin{split}
            Exp \ \textsf{Penalty}(P, \vec{E}) = \int_{Z} \textsf{Penalty}(P, \vec{E}) * F(\vec{E}) \ d\vec{E}
        \end{split}
    \end{equation}
\end{definition}
\textbf{Robustness Metric 1} For a possible plan $P \in \mathbb{P}(Q)$ of the given query $Q$, the robustness value can be measured as the expected cost penalty of that plan based on the distribution of selectivity error and the tolerance threshold $\sigma$
\begin{equation}
\begin{split}
    \mathcal{G}_1(P) \equiv Exp \ \textsf{Penalty}(P, \vec{E})
\end{split}
\end{equation}


\subsection{Robustness Based On Standard Deviation}
\haibo{Maybe move to appendix.} In this specific scenario, two candidate plans may have the same robustness value according to Metric 1. Therefore, we need to define a second metric to help us identify a more stable plan.

\textbf{Robustness Metric 2} For every possible plan $P \in \mathbb{P}(Q)$, we can use the following formula to measure the robustness value based on standard deviation.
\begin{equation}
    \mathcal{G}_2(P) \equiv \sqrt{\int_Z \left[\textsf{Penalty}(P, \vec{E}) - Exp \ \textsf{Penalty}(P, \vec{E})\right]^2 * F(\vec{E})  \ d\vec{E}} 
\end{equation}

\subsection{Robustness Metric Based on the probability of being penalized}

Additionally, to fully understand the robustness of a plan, we also need to know the probability of incurring a penalty. We can use the error distribution to calculate this probability. 

\textbf{Robustness Metric 3} For every possible query plan $P \in \mathbb{P}(Q)$, the robustness metric $\mathcal{G}_3$ is defined as the probability of this plan being penalized with the given threshold,
\begin{equation}
    \begin{split}
        \mathcal{G}_3 \equiv \int_{Z} F(\vec{E}) \ d\vec{E} \quad \text{subject to } \eta > 1 + \sigma.
    \end{split}
\end{equation}
    

The probability of incurring a penalty serves as a guarantee that the plan will be penalized if the error exceeds the tolerance level. This allows us to continue evaluating the robustness of different plans.

\subsection{Find a single robust plan.} 
Given the robustness metrics defined above, our goal is to compute the most robust $P$ in $\mathbb{P}(Q)$ intended for an input selectivity estimated to be $\vec{S}$ with error distribution $\vec{E}$.
\textbf{Dimension Reduction (Only focus on sensitive dimensions)} When calculating robustness metrics, it can be computationally expensive to consider all predicates. For example, there are 13247 dimensions in Q29 of JOB (16-table join query). A large number of predicates makes it more expensive to accurately compute the integral. Therefore, it is necessary to find methods to reduce the dimension. After we have the set of sensitive predicates after the analysis, one way to do this is by focusing on the sensitive predicates, which are the ones that have a significant impact on the cost of the query plan. In this paper, we only use those sensitive dimensions from the entire dimension space and will analyze the effectiveness in terms of the selected plan's performance in the experiment section. \haibo{Modify here: we are not reducing the dimensions, the entire dimensions are the same, we only consider the uncertainty of those sensitive dimensions but remain static for those non sensitive dims.}


\section{Parametric Query Optimization}

Parametric query optimization (PQO) focuses on optimizing parameterized queries, where queries have the same overall SQL structure but vary in the literals of parameters. These queries are frequently executed in modern databases applications and thus provide a significant opportunity to improve their performance. PQO typically involves storing several carefully chosen plans as cached plan candidates. At runtime, the system aims to achieve efficient performance across multiple query instances by selecting a plan from the cached set instead of invoking the optimizer. Each cached plan should be optimal for a subset of all possible values of the runtime parameters \cite{ioannidis1997parametric}. Identifying the appropriate plan should incur a much lower overhead compared with making optimizer call, when the parameters are known for the new query. Unlike the previous work such as \cite{dutt2017leveraging}, which prioritize minimizing sub-optimality in terms of cost, our focus is on demonstrating that the investment in analyzing robust plans can yield substantial benefits. Specifically, we aim to show that SRQO can not only reduce the latency by avoiding calling optimizer, but also deliver efficient execution latency by the robustness of our plan, surpassing the optimal solution achieved by the optimizer at runtime.

Now, the first question arises: for an incoming query with a new parameter combination, how to reuse the cached plans effectively? In the PQO settings, once the original query is analyzed, SRQO stores both the top robust plans and the samples used for their robustness calculation. To avoid calling the optimizer again to calculate the robust plans for the new query, we employ importance sampling \cite{imptsample}. Importance sampling is a Monte Carlo method used to evaluate properties of a target distribution when only samples are available from a different distribution. It helps estimate characteristics of the target distribution by reweighting the samples obtained from the surrogate distribution. For the new query, we assess the estimated robustness of the cached plan by assigning different weights to the penalty values calculated for each sample from the corresponding distribution of the original query. For example, using the expected penalty as an example, the new robustness metrics can be defined as followed.

\begin{definition} \textbf{Expected \textsf{Cost} Penalty by Importance Sampling} For the original query $Q$ with selectivity vector $\vec{S}$, suppose we have $N$ error samples $\{\vec{E_1}, ..., \vec{E_N}\}$ from the original distribution $F(\vec{E})$. For the new query $Q'$ with the selectivity estimation $\vec{S}'$ and the new error distribution $F'(\vec{E})$, the re-weighted expected penalty is defined as:
    \begin{equation} \label{est-exp-cost-penalty}
        \begin{split}
            Exp \ \textsf{Penalty'}(P, \vec{E}) = 
            \frac{1}{N}\sum_{i \in N} \ \textsf{Penalty}(P, \vec{E_i}) * \frac{F'(\vec{E_i'})}{F(\vec{E_i})}
        \end{split}
    \end{equation}
where $\vec{E_i'}$ is the relative error w.r.t $\vec{S'}$, and $\frac{F'(\vec{E_i'})}{F(\vec{E_i})}$ is the weight, representing the ratio of the the probability of $\vec{E_i'}$ being sampled from the new distribution $F'$ to the original distribution. SRQO re-weights the cached samples to estimate the robustness metric for each plan and offer the most robust solution at run-time, without any optimizer's call.
\end{definition}

However, it's essential to acknowledge that relying solely on the robustness analysis of a single query for \textit{all} new queries is unrealistic. We believe that the insights gained from SRQO's robustness analysis are applicable only to specific regions within the overall parameter space. Therefore, only neighboring queries with minimal divergence can effectively benefit from the cached robust plan. For queries exhibiting significant divergence, a large sample size is necessary for accurate estimation. This raises another crucial question: how can we determine whether we can utilize our cached plan for incoming queries at runtime? The lower bound of the sample size required to ensure estimation accuracy through importance sampling is discussed in detail in \cite{2018samplesize}. Typically, the KL-divergence between the new distribution and the original distribution is essential for this determination. We outline the process of examining whether we can reuse the cached plan and the cached samples as follows:
\begin{equation}
\begin{split}
& \text{if } N > \exp\left(KL\left(F(\vec{E}) || F'(\vec{E})\right)\right) \\
& \text{then: Use SRQO cached plans} \\
& \text{else: Use the default optimizer}
\end{split}
\end{equation}

For the incoming query $Q'$, we first calculate the KL-divergence between $F(\vec{E})$ at $\vec{S}$ and $F'(\vec{E})$ at $\vec{S'}$, denoted as $KL(F(\vec{E}) || F'(\vec{E}))$. If the saved sample size is sufficient, we have the guarantee of estimation accuracy and we reuse the samples to calculate the estimated expected cost penalty in \ref{est-exp-cost-penalty}. If the sample size is not enough, we just switch back to the default optimizer.


==> archive/sensitive.tex <==
\section{Sensitive Dimensions} \label{sec: sen-dim}

For each parameterized predicate, we define a sensitivity score that reflects the impact of selectivity uncertainty on that dimension is more likely to cause the original query plan to be sub-optimal. A higher sensitivity score indicates that the selectivity uncertainty has a stronger influence to result in a poor plan choice, while a lower sensitivity score suggests a relatively weaker impact. Those dimensions with high sensitivity scores deserve the administrator to focus more efforts to improve the accuracy and consequently, the responsive optimizer should allow flexible options to the potential uncertainty on those dimensions. \st{The property that the selectivity value for every predicate is independent of each other enables us to evaluate each parameter separately.} In the following section, we will first introduce the method we use to measure the sensitivity of a single dimension and then how to determine the set of dimensions that are sensitive overall.
\subsection{Sensitivity Measurements By Penalty}
To measure the sensitivity of a particular dimension w.r.t a plan, one naive approach is to calculate the slope of the cost function for that dimension. i.e., for a query plan P, the sensitive value to $s_i$ is
$
    \frac{\partial \ \textsf{Cost}(P, \vec{S})}{\partial s_i}
$. The slope determines how sensitive the cost of the plan is to the changes in the selectivity value of that dimension. However, starting from a natural observation that, if the plan is always optimal in the considering area, despite uncertain errors in the selectivity of that dimension, we may still consider this plan insensitive to that dimension even if the cost of the plan changes dramatically. This is because the plan is able to adapt to changes in selectivity without incurring a penalty. So only using the change in cost can not indicate the sensitivity. Instead, we argue that the focus should be on situations where selectivity uncertainty leads the optimizer to choose a sub-optimal plan over the optimal plan, resulting in penalties of cost. Before giving our formal definition of sensitivity we are going to introduce the definition of \textit{cost penalty}. The penalty for a wrong decision is the difference between the estimated cost values of the real optimal plan and the plan that was actually chosen. A small penalty indicates that the plan is acceptable with given uncertainty, while a plan with higher penalty will have lower robustness. On the other hand, a plan that incurs no penalty is robust and able to withstand selectivity errors. Based on this, we propose that a good sensitivity value should focus on the penalty of selecting a poor plan, as determined by the selectivity error. Here, we formally define the concept of \textit{cost penalty}.
\begin{definition}
    \textbf{\textsf{Cost} $\textsf{Penalty}$.} Suppose $P$ is the plan chosen for the point estimates $\vec{S}$. Given $\vec{E}$ as the selectivity error, the corrected selectivity estimates can be regarded as $\vec{S} + \vec{E}$, which is the possible selectivity we are interested in. On this modified selectivity estimate, the optimizer makes another decision $P'$ as the true optimal plan. Then, \textit{penalty} is defined as the cost difference between $P$ and $P'$ on the corrected estimates $\vec{S} + \vec{E}$.
\begin{equation}
\begin{split}
  \textsf{Penalty}(P, \vec{E}) = \textsf{Cost}(P, \vec{S}+\vec{E}) - \textsf{Cost}(P', \vec{S}+\vec{E}) 
\end{split}
\end{equation}
\end{definition} 
$\textsf{Penalty}(\vec{E})$ measures the impact of selectivity errors on query performance when a sub-optimal plan is selected. We further use the definition of penalty to evaluate the \textit{sensitivity} of a predicate to selectivity errors and introduce methods for calculating the sensitivity score. In addition, it may not always be necessary to penalize a plan that is close to optimal. To address this, we can introduce a tolerance factor into the penalty calculation, denoted as $\textsf{Penalty}(\vec{E}, \sigma)$, which represents the maximum cost penalty that we are willing to accept with respect to selectivity uncertainty. If the difference in cost between the selected plan and the optimal plan is within this tolerance, we do not penalize the selected plan. Here we bring the definition of cost penalty with tolerance.
\begin{definition}
    \textbf{\textsf{Cost} Penalty With Tolerance}
    \begin{equation}
    \begin{split}
      \textsf{Penalty}(P, \vec{E}) = 
      \begin{cases}
          0 & \text{ if } \eta \leq 1 + \sigma ,\\
          \textsf{Penalty}(\vec{E}) & \text{ otherwise,}
      \end{cases} 
    \end{split}
\end{equation}
where $\eta$ is the ratio between the cost of the selected plan and the optimal plan, i.e., $\eta = \frac{\textsf{Cost}(P, \vec{S}+\vec{E})}{\textsf{Cost}(P', \vec{S}+\vec{E})}$. $\eta \leq 1 + \sigma$ means the cost of the selected plan is within the tolerance level, so we do not penalize the selected plan, otherwise, we compute $\textsf{Penalty}(\vec{E}, \sigma)$ as before. Incorporating a user-defined tolerance factor into the penalty ensures that we do not unnecessarily penalize plans that are only slightly sub-optimal but still acceptable, enabling us to make more informed and accurate decisions when analyzing the sensitivity to uncertainties.
\end{definition}

\subsection{Global Sensitivity Analysis}
\paragraph{\textbf{Local Sensitivity Method}}

Previous approaches in sensitivity analysis \cite{2018rqo} often involved computing the slope of the cost function for each dimension at the local point-wise selectivity estimation and utilizing the "one-at-a-time" (OAT) technique, perturbing only one dimension at a time while keeping others static. Using the penalty measurement in the parametric query optimization settings, the local sensitivity of a parameter can be defined.
\begin{definition}
    \textbf{Local Sensitivity by Penalty}
    Use $\Delta e_i$ to denote the perturbation,
    \begin{equation}
    \begin{split}
        SA_i^{local} &= \frac{\partial \ \textsf{Penalty}(P, \vec{E})}{\partial e_i} \\  
        &= \frac{\textsf{Penalty}(P, \vec{E} + \Delta e_i) - \textsf{Penalty}(P, \vec{E})}{\Delta e_i}
    \end{split}
    \end{equation}
where $\vec{E} + \Delta e_i = \{e_1, ..., e_i+\Delta e_i, ..., e_{d}\}$ \haibo{Reduce (6) to 1 line maybe}.
\end{definition}
For a given $P$, $SA_i^{local}$ can be calculated efficiently, since we only need $d+1$ simulations to calculate the differences of penalty. However, OAT at local has clear drawbacks. It relies on delicate and singular point selectivity estimates, lacking a global sensitivity analysis perspective. Furthermore, it focuses solely on individual parameters, overlooking potential interactions among them, which can lead to significant output variance.
\paragraph{\textbf{Morris}}
To address these limitations, our first objective is to shift from local to global sensitivity analysis. The Morris method \cite{morris1991factorial} presents a more comprehensive approach in this regard. Serving as an extension of traditional local sensitivity analysis \cite{wainwright2014making}, Morris draws $K$ samples from input parameters' space, and for each sample, applies OAT perturbations to each dimension. To be specific, Morris begins with a random order of the dimensions, following this order to determine the direction of perturbation. It captures the output variation of each dimension when perturbed individually, while keeping previously perturbed dimensions static. The final sensitivity of each dimension is calculated by averaging these variations across all samples. The Morris method goes beyond the constraints of local sensitivity analysis by performing partial derivative calculations at diverse points within the input variable domain of variation, thereby achieving a global perspective a global scope, enabling the input variables to span their entire domain of definition. In the context of SRQO, where the distribution of $F(\vec{E})$ is given, we employ the penalty measurement to define Morris sensitivity.

\begin{definition}
    \textbf{Morris Sensitivity by Penalty} ${\vec{E_k}} = \{ e_1, e_2, ..., e_d \}$ is one of $K$ samples from $F(\vec{E})$, while $\vec{E_k^{\ast}} = \{ e_1^{\ast}, e_2^{\ast}, ..., e_d^{\ast} \}$ represents the current state after previous perturbations, following the generated order of dimensions. The current perturbation is $\Delta e_i^{\ast}$,
    
    \begin{equation}
    \begin{split}
        SA_i^{Morris} &= Avg \ \frac{\partial \ \textsf{Penalty}(P, \vec{E_k^{\ast}})}{\partial e_i^{\ast}}  \\ 
        &= Avg \ \frac{\textsf{Penalty}(P, \vec{E_k^{\ast}} + \Delta e_i^{\ast}) - \textsf{Penalty}(P, \vec{E_k^{\ast}})}{\Delta e_i^{\ast}} 
    \end{split}
    \end{equation}

where $\vec{E_k^{\ast}} + \Delta e_i^{\ast} = \{e_1^{\ast}, ..., e_i^{\ast}+\Delta e_i^{\ast}, ..., e_{d}^{\ast}\}$.
\end{definition}

For $K$ samples, Morris requires $K\*(d+1)$ simulations to calculate the variance of the output. Despite its global perspective, the Morris method is not designed to discriminate between the effects of parameter interactions, presenting a limitation in discerning individual parameter impacts in certain scenarios. We introduce another method which fully consider the interactions between parameters.
\paragraph{Sobols} In a global sensitivity analysis, all parameters are simultaneously varied across the entire parameter space. Sobol's method \cite{SOBOL2001271} enables the simultaneous evaluation of the relative contributions of each individual parameter as well as the interactions between parameters to the variance of the model output. This method decomposes the variance of the model output into components attributed to the variance of individual parameters, combined effects of parameter pairs, and so on. Sobols sensitivity analysis aims to quantify the extent to which variations in model output are influenced by individual input parameters or interactions between them.

Considering the broad range of model inputs and the error distribution of different predicates, Sobols method emerges as an innovative method for identifying the primary contributors to the overall system behavior among reactions and processes.





\haibo{Maybe skip this: Use query 17 and it's recentered plan, and then show the sensitive dimensions and explain why}

\haibo{\textbf{maybe add how we "build plan pool" and "reduce dims" here? since we just have the sensitive dim}}



==> temp.tex <==
\begin{table}[t]
\begin{small}
    
    \centering
    \begin{tabular}{ccccc}
    \toprule
        Q ID & \# of table & \# of LSC & d & Sensitive Dim \\ \midrule
        q2 & 5 & 2 & 7 & mc-cn, cn, k, mk-k,  \\
        q17 & 7 & 3 & 12 & mk-k \\ 
        q15 & 9 & 5 & 19 & t-akat, mc, mc-cn \\
        q26 & 12 & 8 & 24 & miidx-it, t-cc, miidx \\
        \bottomrule
    \end{tabular}
\end{small}
    \caption{Information of Queries \haibo{This table is useless if we have Figure \ref{fig:graph}}}
    \label{tab:basic_info}
\end{table}




\begin{table*}[htbp]
\begin{small}
    
\centering
\label{tab:summary}
\begin{tabular}{@{}ccccccc@{}}
\toprule
Q ID & \# of parameters & \# of satisfied Q & \# of Q cached is faster & AVG robust (ms) & AVG pg (ms) & Ratio \\ \midrule
1 & 3 & 55/100 & 51/55 & 153 & 311 & 103\% \\
2 & 2 & 36/100 & 26/36 & 129 & 193  & 50\% \\
3 & 3 & 53/100 & 14/53 & 171 & 165  & -3.6\% \\
4 & 4 & 25/100 & 7/25 & 149 & 133  & -12\% \\
5 & 4 & 16/100 & 9/16 & 95.7 & 96.5  & 1\% \\
6 & 3 & 8/100 & 6/8 & 341 & 512  & 50\% \\
7 & 7 & 47/100 & 16/41 & 81 & 126  & 56\% \\
8 & 5 & 14/100 & 6/14 & 154 & 359  & 133\% \\
9 & 6 & 9/100 & 7/9 & 110 & 111  & 1\% \\
10 & 4 & 1/100 & 1/1 & 655  & 655 & 0 \\
11 & 6 & 15/100 & 13/15 & 20.44 & 43.46  & 113\% \\
12 & 6 & 46/100 & 26/46 & 338 & 353  & 4\% \\
13 & 5 & 85/100 & 44/85 & 1077 & 1221 & 13\% \\
14 & 7 & 26/100 & 16/26 & 233 & 231  & -0.86\% \\
15 & 5 & 2/100 & 1/2 & 168 & 186  & 10\% \\
16 & 3 & 16/100 & 7/16 & 1190  & 1190 & 0 \\
17 & 3 & 74/100 & 65/74 & 836 & 5466  & 554\% \\
18 & 4 & 36/100 & 34/36 & 107 & 3157  & 2827\% \\
19 & 8 & 6/100 & 3/6 & 104 & 105  & 0.8\% \\
20 & 5 & 12/100 & 7/12 & 117 & 206  & 76\% \\
21 & 7 & 11/100 & 10/11 & 20.35 & 46.98  & 131\% \\
22 & 8 & 15/100	& 10/15 & 88 & 106 & 20\% \\
23 & 6 & 15/100 & 9/15 & 91 & 92  & 1.1\% \\
24 & 8 & 2/100 & 2/2 & 96.25 & 101.1  & 5\% \\
25 & 6 & 3/100 & 3/3 & 231 & 987  & 326\% \\
26 & 8 & 9/100 & 7/9 & 254 & 707  & 178\% \\
27 & 9 & 11/100 & 1/11 & 5.9 & 5.9 & 0 \\
28 & 11 & 23/100 & 13/23 & 149 & 242  & 62\% \\
29 & 12 & 2/100 & 2/2 & 53.9 & 66.2  & 23\% \\
30 & 9 & 41/100 & 32/41 & 101 & 363  & 253\% \\
31 & & & & & & \\
32 & 1 & 62/100 & 43/62 & 26.7 & 34.1  & 28\% \\
33 & & & & & &  \\ \bottomrule
\end{tabular}
\caption{Summary of PQO Results}
\label{pqo}
\end{small}

\end{table*}


Here, we formally define the concept of \textit{cost penalty}.
\begin{definition}
    \textbf{\textsf{Cost} $\textsf{Penalty}$.} Suppose $P$ is the plan chosen for the point estimates $\vec{S}$. Given $\vec{E}$ as the selectivity error, the corrected selectivity estimates can be regarded as $\vec{S} + \vec{E}$, which is the possible selectivity we are interested in. On this modified selectivity estimate, the optimizer makes another decision $P'$ as the true optimal plan. Then, \textit{penalty} is defined as the cost difference between $P$ and $P'$ on the corrected estimates $\vec{S} + \vec{E}$.
\begin{equation}
\begin{split}
  \textsf{Penalty}(P, \vec{E}) = \textsf{Cost}(P, \vec{S}+\vec{E}) - \textsf{Cost}(P', \vec{S}+\vec{E}) 
\end{split}
\end{equation}
\end{definition} 
$\textsf{Penalty}(\vec{E})$ measures the impact of selectivity errors on query performance when a sub-optimal plan is selected. We further use the definition of penalty to evaluate the \textit{sensitivity} of a predicate to selectivity errors and introduce methods for calculating the sensitivity score. In addition, it may not always be necessary to penalize a plan that is close to optimal. To address this, we can introduce a tolerance factor into the penalty calculation, denoted as $\textsf{Penalty}(\vec{E}, \sigma)$, which represents the maximum cost penalty that we are willing to accept with respect to selectivity uncertainty. If the difference in cost between the selected plan and the optimal plan is within this tolerance, we do not penalize the selected plan. Here we bring the definition of cost penalty with tolerance.
\begin{definition}
    \textbf{\textsf{Cost} Penalty With Tolerance}
    \begin{equation}
    \begin{split}
      \textsf{Penalty}(P, \vec{E}) = 
      \begin{cases}
          0 & \text{ if } \eta \leq 1 + \sigma ,\\
          \textsf{Penalty}(\vec{E}) & \text{ otherwise,}
      \end{cases} 
    \end{split}
\end{equation}
where $\eta$ is the ratio between the cost of the selected plan and the optimal plan, i.e., $\eta = \frac{\textsf{Cost}(P, \vec{S}+\vec{E})}{\textsf{Cost}(P', \vec{S}+\vec{E})}$. $\eta \leq 1 + \sigma$ means the cost of the selected plan is within the tolerance level, so we do not penalize the selected plan, otherwise, we compute $\textsf{Penalty}(\vec{E}, \sigma)$ as before. Incorporating a user-defined tolerance factor into the penalty ensures that we do not unnecessarily penalize plans that are only slightly sub-optimal but still acceptable, enabling us to make more informed and accurate decisions when analyzing the sensitivity to uncertainties.
\end{definition}




\subsection{Problem Defnination}
To formally define the problem, let's consider a query $Q$ with a set of $d$ parameterized selectivity values. These selectivity values can be represented as a point in a $d$-dimensional space, denoted by $\vec{S} = \{ s_1, s_2, ..., s_d\}$. Each value $s_i$ indicates the proportion of rows in a table or join that satisfy the corresponding predicate. For each possible execution plan $P$ of $Q$, the optimizer uses a parameterized cost function to evaluate its efficiency. The cost function takes the potential plan $P$ and the selectivity combination $\vec{S}$ as the input parameters and returns the estimated cost (without execution) of $P$, notated as  $\textsf{Cost}(P, \vec{S})$. The cost function has the same dimension as the number of selectivity parameters. The physical plans we are considering are with different join orders, join methods and scan methods. We leverage the existing cost-based query optimizer to calculate the value and regard the cost model as a black box since the function is complex and opaque to the parameters. Following the assumption in several previous works (plan bouquets serious), we also assume this cost value can be precisely calculated by the cost model. Our experiment also demonstrated that there is a strong correlation between the cost model and the running time, which is consistent with \cite{job}.


\begin{definition} Given a query $Q$, let $\mathbb{P}(Q)$ be the set of all possible execution plans. Then, the optimizer will search for the one in $\mathbb{P}(Q)$ with the minimum cost, 
\begin{equation}
     \arg \min_{P \in \mathbb{P}(Q)} \textsf{Cost}(P, \vec{S})
\end{equation}
and return it for the user to execute. 

However, due to the limited learnability of current selectivity estimation models, it is hard to accurately estimate the selectivity value. The errors contained in cardinalities might result in the plan chosen by the optimizer being sub-optimal or even poor. Given the truth that the error of estimations is unavoidable, we claim to make the optimizer aware of the selectivity uncertainties and then select the most robust plan based on the potential errors instead of the point estimates only.
\end{definition}
\begin{definition}
Suppose $\vec{E} = \{ e_1, e_2, ..., e_d\}$ is the potential selectivity errors on each dimension in $\vec{S}$. To capture the error distribution of each dimension, we define $F(\vec{E})$ as the joint probability density function (PDF) of potential errors $\vec{E}$. $F(\vec{E}) = \prod_{i=1}^{d} f_{i}(e_{i})$, where $f_{i}(e_{i})$ is the PDF of selectivity error on dimension $i$. $F(\vec{E})$ can describe the joint distribution of the selectivity error on $d$ predicates, and the boundary of this error distribution is a hyper-rectangle with $d$ dimensions, notated as $\mathbf{Z}$, i.e, $\vec{E} \in \mathbf{Z}$. The following conditions must be satisfied:

\begin{equation}
    \forall i \in [0, d], f_{i}(e_i) > 0 \text{, and} \int_{\mathbf{Z}_{i}} f_{i}(e_{i}) \ de_{i} = 1\\
\end{equation}
\begin{equation}
    \forall \vec{E} \in \mathbf{Z}, F(\vec{E}) > 0 \text{, and} \int_{\mathbf{Z}} F(\vec{E}) \ d\vec{E} = 1\\
\end{equation}
The distribution of selectivity errors allows us to quantify uncertainties, and our ultimate goal is to make the optimizer aware of these uncertainties and select a plan that is resilient to such errors. Section \ref{sec: err} will introduce how we collect the real error data from the historical executions and how to build the error distribution. In this paper, we are particularly interested in understanding and identifying those critical components where uncertainties can significantly impact the final performance and plan choice. We refer to these critical components of the query as "sensitive dimensions" that require extra attention and effort to ensure a robust outcome.


\end{definition}



\begin{table*}[t]
% \setlength{\tabcolsep}{8.9pt}
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Base Tables} & \textbf{2-tables Join} & \textbf{3-tables Join} & \textbf{4-tables Join} & \textbf{5 to 7 tables Join} \\
    ci & (mc ci) & (cn ci mc) & (mk ci cn mc) & (k ci cn mc mk)\\
    cn & (mk ci) & (mk ci mc) & (n ci cn mc) & (n ci cn mc mk) \\
    k & (n ci) & (n ci mc) & (k ci mc mk) & (t ci cn mc mk) \\
    mc & (t ci) & (t ci mc) & (n ci mc mk) & (t ci cn mc n) \\
    mk & (mc cn) & (k ci mk) & (t ci mc mk) & (n ci k mc mk) \\
    n & (mk k) & (n ci mk) & (n ci k mk) & (t ci k mc mk) \\
    t & (mk mc) & (t ci mk) & ... & ... \\
     & (t mc) & (t ci n) & ... & ... \\
     &  & (mk cn mc) & ... & ... \\
  &  & (t cn mc) & ... & ... \\
   &  & (mc k mk) & ... & ... \\
    &  & (t k mk) & ... & ... \\
  &  & (t mc mk) & ... & ... \\
    7 dims & 9 dims & 13 dims & 13 dims & 14 dims \\
\hline
\end{tabular}

\caption{Dimension Categories in Q17. In total, we have 56 dims. Each is a dimension in the cost function.}
\label{tab: q17-ori-dim}
\end{table*}



\begin{table}[]
\begin{small}
\centering
\begin{tabular}{p{0.7cm}p{0.8cm}p{1.0cm}p{0.9cm}p{0.9cm}p{0.9cm}p{0.8cm}}
\hline
& Movie & TV \hspace{0.3cm} Series & TV Movie & Video Movie & Video Game & Episode \\
\hline
 t & 663k & 91k & 101k & 118k & 13k & 1543k \\
 mc & 1308k & 194k & 200k & 160k & 30k & 717k \\
 mk & 2887k & 183k & 251k & 473k & 85k & 645k \\
 ci & 10397k & 889k & 1950k & 1378k & 211k & 21420k \\
 % ml & 0 & 12k & 0 & 0 & 0 & 18k \\
 mi & 8301k & 770k & 804k & 883k & 115k & 3963k \\
 cc & 60k & 3k & 8k & 3k & 65 & 62k \\
 at & 293k & 20k & 27k & 13k & 5k & 3k \\
 miidx & 630k & 113k & 111k & 84k & 17k & 426k \\
 k & 111k & 25k & 34k & 27k & 12k & 65k \\
 cn & 188k & 31k & 28k & 27k & 5k & 12k \\
 % an & 637k & 87k & 150k & 106k & 12k & 290k \\
 n & 637k & 87k & 150k & 106k & 12k & 290k \\
 % pi & 748k & 363k & 526k & 338k & 78k & 644k \\
 % lt & 0 & 16 & 0 & 0 & 0 & 15 \\
 it & 95 & 92 & 92 & 93 & 53 & 57 \\
 ct & 2 & 2 & 2 & 2 & 2 & 2 \\
 kt & 1 & 1 & 1 & 1 & 1 & 1 \\
 chn & 1699k & 164k & 370k & 132k & 41k & 1185k \\
 % rt & 11 & 11 & 11 & 11 & 11 & 11 \\
 cct & 4 & 4 & 4 & 4 & 3 & 4 \\
\hline
\end{tabular}

\caption{\small{Information of DB instances partitioned by \textit{kind\_type.kind} on \textit{item} to imitate the unknown selectivity errors in the practical situation. We omit other tables that are not involved in representative queries Q2, Q17, Q26, and Q15.}}
\label{tab:cat}
\end{small}

\end{table}




\subsection{Robustness Based On Expected \textsf{Cost} Penalty}
A recently proposed robustness metrics \cite{2018rqo} typically evaluate the behavior of a plan by only analyzing the slope and integral of the cost function. However, these approaches may not always provide sufficient information to accurately assess the robustness of a plan. \haibo{Do we need a x-y 2-d plot here?} shows that the slope or integral of the cost function as the robustness value can not reflect if the plan is more robust than the other. Instead, we believe that robustness evaluation should focus on how \textit{poorly} a plan could perform. Likewise, even if the selected plan is not optimal, we may still consider it if its performance is not significantly worse. Therefore, to better understand plan robustness, it is more effective to identify the region where a wrong plan decision, as determined by the selectivity error, results in a penalty. Using a similar idea when we analyze the sensitive predicates, our first robustness metric is defined as the expected cost penalty using the selectivity error distribution.
\begin{definition} \textbf{Expected \textsf{Cost} Penalty} The expected cost penalty over the joint selectivity error distribution w.r.t the tolerance threshold is
    \begin{equation}
        \Expectation[\Penalty(\plan, \Sels) | \hat \sels] = \int \Penalty(\plan, \sels) \cdot f(\sels | \hat \sels) \di \sels
    \end{equation}
\end{definition}
\textbf{Robustness Metric 1} For a possible plan $\plan \in \PlanSpace(Q)$ of the given query template $Q$ with selectivity estimate $\hat \sels$, the robustness value can be measured as the expected cost penalty of that plan based on the distribution of selectivity error and the tolerance threshold $\tau$
\begin{equation}
\begin{split}
    \mathcal{G}_1(\plan) \equiv \Expectation[\Penalty(\plan, \Sels) | \hat \sels]
\end{split}
\end{equation}


\subsection{Robustness Based On Standard Deviation}
\haibo{Maybe move to appendix.} In this specific scenario, two candidate plans may have the same robustness value according to Metric 1. Therefore, we need to define a second metric to help us identify a more stable plan.

\textbf{Robustness Metric 2} For every possible plan $\plan \in \PlanSpace(Q)$, we can use the following formula to measure the robustness value based on standard deviation.
\begin{equation}
    \mathcal{G}_2(\plan) \equiv \sqrt{\int \left[\Penalty(\plan, \sels) - \mathcal{G}_1(\plan)\right]^2 * f(\sels | \hat \sels) \di \sels} 
\end{equation}

\subsection{Robustness Metric Based on the probability of being penalized}

Additionally, to fully understand the robustness of a plan, we also need to know the probability of incurring a penalty. We can use the error distribution to calculate this probability. 

\textbf{Robustness Metric 3} Given $\plan \in \PlanSpace(Q)$, the robustness metric $\mathcal{G}_3$ is defined as the probability of $\plan$ being penalized with the given threshold $\tau$,
\begin{equation}
    \begin{split}
        \mathcal{G}_3(\plan) \equiv \int f(\sels | \hat \sels) \di \sels \quad \text{subject to } \Cost(\plan, \sels) > (1 + \tau) \cdot \optCost(\sels),.
    \end{split}
\end{equation}
    

The probability of incurring a penalty serves as a guarantee that the plan will be penalized if the error exceeds the tolerance level. This allows us to continue evaluating the robustness of different plans.

Furthermore, we eliminate corner cases where certain combinations of predicate literals yield nonsensical results, such as instances where the output of a combination produces zero rows. When processing a query, if the optimizer detects a relation producing zero rows, it typically avoids executing subsequent join relations, thus saving execution time. Therefore, the execution time becomes uncorrelated from the estimated cost. Additionally, when a query plan is hinted, the optimizer is compelled to follow the hinting, regardless of whether there is a zero rows of relation. Consequently, we are unable to monitor the end-to-end behaviors of plan candidates in a fair manner.


This decision is informed by the understanding that PARQO's analysis of the original query is applicable primarily to its neighboring queries. Given that only a small region of the query space benefits from robustness, storing a few plans is sufficient to maintain efficiency and effectiveness in handling similar queries.
